Cloud-Device Collaborative Agents for Sequential Recommendation

Recent advances in large language models (LLMs) have enabled agent-based recommendation systems with strong semantic understanding and flexible reasoning capabilities. While LLM-based agents deployed in the cloud offer powerful personalization, they often suffer from privacy concerns, limited access to real-time signals, and scalability bottlenecks. Conversely, on-device agents ensure privacy and responsiveness but lack the computational power for global modeling and large-scale retrieval. To bridge these complementary limitations, we propose CDA4Rec, a novel Cloud-Device collaborative framework for sequential Recommendation, powered by dual agents: a cloud-side LLM and a device-side small language model (SLM). CDA4Rec tackles the core challenge of cloud-device coordination by decomposing the recommendation task into modular sub-tasks including semantic modeling, candidate retrieval, structured user modeling, and final ranking, which are allocated to cloud or device based on computational demands and privacy sensitivity. A strategy planning mechanism leverages the cloud agent's reasoning ability to generate personalized execution plans, enabling context-aware task assignment and partial parallel execution across agents. This design ensures real-time responsiveness, improved efficiency, and fine-grained personalization, even under diverse user states and behavioral sparsity. Extensive experiments across multiple real-world datasets demonstrate that CDA4Rec consistently outperforms competitive baselines in both accuracy and efficiency, validating its effectiveness in heterogeneous and resource-constrained environments.

==> deleted.tex <==
% \paragraph{Accuracy.}
% The adaptive CDARA model consistently achieves the highest HR@10 among all versions. This confirms the benefit of context-aware strategy planning in selecting appropriate modeling techniques based on user intent, behavior sparsity, and query specificity. In contrast, most fixed-strategy variants (e.g., $v_1$, $v_2$, $v_4$) exhibit significantly lower accuracy, indicating that static configurations fail to generalize well across heterogeneous user scenarios. Notably, variants such as $v_7$ (replacing SASRec with TGCL4SR) and $v_8/v_9$ (altering the ranking weight $\beta$) help identify components most sensitive to strategic decisions, offering useful insights into module-level contribution.

% \paragraph{Latency.}
% While the adaptive pipeline introduces a slight overhead due to runtime strategy inference, its end-to-end recommendation latency remains comparable to most fixed baselines and significantly lower than LSC4Rec. This suggests that CDARA’s dynamic planning mechanism is lightweight enough to be deployed in practical settings without sacrificing responsiveness.

% \paragraph{Communication Cost.}
% CDARA achieves a favorable trade-off between accuracy and communication efficiency. The strategy planner allows selective module offloading, which reduces redundant parameter transmission. Compared to LSC4Rec, CDARA achieves better accuracy with a smaller or comparable communication cost, demonstrating its superior cost-effectiveness. Among the fixed variants, $v_4$ and $v_9$ reduce communication cost the most due to smaller candidate pools or disabled ranking modules, but at the cost of significant accuracy drops.

% \paragraph{Overall Findings.}
% These results validate that adaptive strategy planning is a key enabler of personalization and efficiency in cloud-device collaborative recommendation. It dynamically balances semantic and structured modeling, adjusts candidate scale, and tunes ranking importance according to user context. Compared with static pipelines and lightweight baselines, CDARA achieves a more desirable balance between recommendation quality, latency, and communication overhead.




% These evaluations collectively assess the recommendation quality, adaptability, and system efficiency brought by strategy planning in CDARA.




% We evaluate each version in terms of \textbf{recommendation accuracy} (HR@K and NDCG@K), \textbf{recommendation latency}, and \textbf{communication cost} (i.e., the amount of parameters uploaded and downloaded between device and cloud). We also include \textbf{LSC4Rec} as a lightweight baseline for comparison. These evaluations collectively assess the recommendation quality, adaptability, and system efficiency brought by strategy planning in CDARA.



% The motivation lies in the observation that users exhibit diverse behaviors and query intents, which require different recommendation strategies. Rigid, fixed pipelines may fail to capture such variability, leading to sub-optimal recommendation performance and inefficient resource usage.

% We compare the full CDARA system---which dynamically selects module configurations based on user context---with ten fixed-strategy baselines, denoted as $v_1$ to $v_{10}$. Each baseline applies a static setting to the four core components of the pipeline: \textit{Semantic User Modeling}, \textit{Candidate Retrieval}, \textit{Structured User Modeling}, and \textit{Final Ranking}. The ablation settings for each version are summarized in Table~\ref{tab:cdara_ablation}.


% In addition to measuring top-$K$ recommendation accuracy (HR@K and NDCG@K), we also evaluate each version's \textbf{recommendation latency}, \textbf{communication cost} (i.e., upload and download parameter size between device and cloud), and compare against a recent lightweight framework \textbf{LSC4Rec}. These evaluations help assess not only the recommendation quality, but also the adaptability and efficiency enabled by strategy planning in CDARA.











% Dataset
% music + movie + sport + POI

% Baselines
% Centralized
% lightgcn
% GRU4Rec
% SASRec
% P5
% RAREC


% Cloud-device Collaborative
% LSC4Rec
% DCCL
% MetaController
% DUET

% 1. recommendation accuracy
% 2. recommendation efficiency
% training time
% inference time
% communication






% 1.recommendation accuracy
% 2.efficiency - save time and trans communication 
% 3.可解释性 - 如何判断可解释性呢？人为
% 4. case study
% 5 adapter
% 4.ablation study
% Analysis of the influence of item popularity
% Analysis of the influence of domain
% The influence of strategy-level suggestions strategy vs no strategy
% The impact of choosing different LLMs on performance.
% The impact of choosing different SRMs on performance.
%  Analysis of resource consumption.
%   The impact of length of candidate list


% In this section, we perform comprehensive experiments with two real-world datasets to evaluate the effectiveness and efficiency of the proposed DCPR. The comparative analysis includes two categories of baselines: centralized POI recommendation systems and on-device POI recommenders. Specifically, our investigation seeks to address the following research questions:

% \noindent{\textbf{RQ1}}: How does the DCPR perform compared with state-of-the-art POI recommendation methods?

% \noindent{\textbf{RQ2}}: How does the cloud-device collaboration contribute to performance and efficiency?

% \noindent{\textbf{RQ3}}: strategy vs fixed

% \noindent{\textbf{RQ4}}: Is CDARA capable of generating meaningful explanations on-device?

% \begin{table*}[t]
% \centering
% \caption{Dataset Statistics}
% \begin{tabular}{lccccc}
% \toprule
% \textbf{Domain} & \textbf{POI} & \textbf{Music} & \textbf{Book} & \textbf{Movie} & \textbf{Sport} \\
% \textbf{Dataset} & Foursquare\_NYC & Music4All & BX & MovieLens-10M & Amazon-Sport \\
% \midrule
% \#User & 1{,}083 & 14{,}127 & 278{,}858 & 71{,}567 & 4{,}663{,}297 \\
% \#Item & 38{,}333 & 109{,}269 & 271{,}379 & 10{,}681 & 781{,}509 \\
% \#Interactions & 227{,}428 & 5{,}109{,}592 & 1{,}031{,}176 & 10{,}000{,}054 & 8{,}351{,}612 \\
% \#Item per user & 210.00 & 361.69 & 3.70 & 139.73 & 1.79 \\
% \bottomrule
% \end{tabular}
% \label{tab:dataset_stats}
% \end{table*}


% \begin{table*}
% \centering
% \caption{Performance comparison between CCMPR, P5, and GPT4Rec across five domains.}
% \label{performance}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lrrrrrrrrrrrrrrrrrrrr}
% \toprule
% {} & \multicolumn{4}{c}{POI} & \multicolumn{4}{c}{Music} & \multicolumn{4}{c}{Book} & \multicolumn{4}{c}{Movie} & \multicolumn{4}{c}{Sport} \\
% {} &  HR@10 &  HR@50 & HR@100 & NDCG@10 &  HR@10 &  HR@50 & HR@100 & NDCG@10 &  HR@10 &  HR@50 & HR@100 & NDCG@10 &  HR@10 &  HR@50 & HR@100 & NDCG@10 &  HR@10 &  HR@50 & HR@100 & NDCG@10 \\
% Model   &        &        &        &         &        &        &        &         &        &        &        &         &        &        &        &         &        &        &        &         \\
% \midrule
% CCMPR   & 0.0851 & 0.1249 & 0.1437 &  0.0642 & 0.0904 & 0.1295 & 0.1476 &  0.0695 & 0.0376 & 0.0542 & 0.0615 &  0.0281 & 0.0763 & 0.1127 & 0.1324 &  0.0573 & 0.0248 & 0.0347 & 0.0410 &  0.0172 \\
% P5      & 0.0732 & 0.1060 & 0.1151 &  0.0530 & 0.0820 & 0.1108 & 0.1201 &  0.0583 & 0.0334 & 0.0465 & 0.0502 &  0.0248 & 0.0650 & 0.0923 & 0.1041 &  0.0453 & 0.0211 & 0.0276 & 0.0317 &  0.0145 \\
% GPT4Rec & 0.0653 & 0.0975 & 0.1090 &  0.0486 & 0.0714 & 0.0997 & 0.1122 &  0.0501 & 0.0297 & 0.0411 & 0.0455 &  0.0211 & 0.0556 & 0.0809 & 0.0912 &  0.0390 & 0.0180 & 0.0245 & 0.0279 &  0.0122 \\
% \bottomrule
% \end{tabular}}
% \end{table*}


% \begin{table*}[t]
% \centering
% \caption{Performance comparison across datasets and methods}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccccccccccccc}
% \toprule
% \textbf{Method} & \multicolumn{4}{c}{\textbf{Movie}} & \multicolumn{4}{c}{\textbf{Music}} & \multicolumn{4}{c}{\textbf{Sports}} & \multicolumn{4}{c}{\textbf{POI}} \\
% & HR@5 & NDCG@5 & HR@10 & NDCG@10 & HR@5 & NDCG@5 & HR@10 & NDCG@10 & HR@5 & NDCG@5 & HR@10 & NDCG@10 & HR@5 & NDCG@5 & HR@10 & NDCG@10 \\
% \midrule
% \multicolumn{17}{c}{\textit{Cloud-side Inference}} \\
% GRU4Rec & 0.0111 & 0.0069 & 0.0199 & 0.0099 & 0.0105 & 0.0061 & 0.0185 & 0.0086 & 0.0089 & 0.0053 & 0.0162 & 0.0077 & 0.2536 & 0.1876 & 0.3615 & 0.2177 \\
% SASRec & 0.0143 & 0.0085 & 0.0256 & 0.0131 & 0.0132 & 0.0079 & 0.0233 & 0.0108 & 0.0101 & 0.0067 & 0.0191 & 0.0094 & 0.2614 & 0.1967 & 0.3741 & 0.2293 \\
% SR-GNN & 0.0181 & 0.0111 & 0.0305 & 0.0159 & 0.0156 & 0.0092 & 0.0263 & 0.0123 & 0.0118 & 0.0072 & 0.0207 & 0.0106 & 0.2955 & 0.2150 & 0.3976 & 0.2485 \\
% RARec & 0.0235 & 0.0166 & 0.0394 & 0.0240 & 0.0233 & 0.0155 & 0.0388 & 0.0229 & 0.0128 & 0.0090 & 0.0230 & 0.0125 & 0.3220 & 0.2328 & 0.4489 & 0.2669 \\
% \midrule
% \multicolumn{17}{c}{\textit{Device-side Inference}} \\
% LLRec & 0.0099 & 0.0059 & 0.0177 & 0.0085 & 0.0091 & 0.0053 & 0.0163 & 0.0076 & 0.0079 & 0.0046 & 0.0145 & 0.0066 & 0.2216 & 0.1613 & 0.3073 & 0.1950 \\
% PREFER & 0.0103 & 0.0065 & 0.0183 & 0.0092 & 0.0098 & 0.0058 & 0.0174 & 0.0081 & 0.0083 & 0.0050 & 0.0151 & 0.0070 & 0.2392 & 0.1768 & 0.3392 & 0.1974 \\
% \midrule
% \multicolumn{17}{c}{\textit{Cloud-device Collaborative Inference}} \\
% DCCL & 0.0145 & 0.0086 & 0.0264 & 0.0133 & 0.0134 & 0.0081 & 0.0239 & 0.0111 & 0.0103 & 0.0068 & 0.0193 & 0.0095 & 0.2621 & 0.2019 & 0.3796 & 0.2360 \\
% DUET & 0.0172 & 0.0107 & 0.0285 & 0.0149 & 0.0148 & 0.0087 & 0.0252 & 0.0115 & 0.0109 & 0.0069 & 0.0195 & 0.0102 & 0.2872 & 0.2094 & 0.3908 & 0.2422 \\
% LSC4Rec & 0.0242 & 0.0170 & 0.0401 & 0.0253 & 0.0242 & 0.0164 & 0.0396 & 0.0236 & 0.0133 & 0.0094 & 0.0236 & 0.0130 & 0.3290 & 0.2387 & 0.4607 & 0.2799 \\
% Our Method & 0.0259 & 0.0182 & 0.0423 & 0.0271 & 0.0256 & 0.0178 & 0.0426 & 0.0250 & 0.0176 & 0.0121 & 0.0275 & 0.0174 & 0.3589 & 0.2576 & 0.4845 & 0.3046 \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:method_comparison}
% \end{table*}

% \begin{table}[ht]
% \centering
% \caption{Inference Time Comparison (ms/sample) Across Domains}
% \begin{tabular}{lcccc}
% \toprule
% \textbf{Model} & \textbf{Movie} & \textbf{Music} & \textbf{Sports} & \textbf{POI} \\
% \midrule
% RARec      & 493.18  & 1072.94 & 392.73 & 235.01 \\
% TransRec   & 501.91  & 1115.98 & 411.13 & 248.04 \\
% LSC4Rec    & 677.16  & 1500.72 & 531.32 & 325.05 \\
% CDARA      & \textbf{88.95}   & \textbf{93.41}   & \textbf{70.48}  & \textbf{42.61} \\
% \bottomrule
% \end{tabular}
% \label{tab:inference_time}
% \end{table}

\subsection{Effect of Different Trajectory Length (RQ4)}

\subsection{Hyperparameter Sensitivity (RQ5)}

In POI recommendation, the length of a user's check-in trajectory significantly impacts recommendation accuracy, making it crucial for a recommender system to maintain robustness across varying sequence lengths. To systematically assess this effect, we categorize users’ check-in sequences into three groups: short (fewer than 50 check-ins), medium (50–200 check-ins), and long (more than 200 check-ins). We compare the performance of four models, including Mobility-LLM-large, which serves as the strongest baseline, and our proposed models TZPR-Small, TZPR-Medium, and TZPR-Large. The results are presented in Figure \ref{Fig:edtl}, using HR@10 as the evaluation metric. %The results, recorded in Figure \ref{Fig:edtl}, use HR@10 as the evaluation metric.


As expected, a general trend emerges across all datasets: as the length of a user’s check-in sequence increases, the model gains a richer understanding of their preferences, leading to improved recommendation accuracy. This highlights the advantage of longer historical data in capturing user behaviors more comprehensively. However, despite this overall trend, Mobility-LLM-large exhibits a noticeable limitation: while its performance is relatively strong for short and medium-length sequences, it stagnates or shows minimal improvement when dealing with long trajectories. This is likely due to interest drift, where users’ preferences shift over time, making it challenging for the model to maintain stable representations over extended periods. Additionally, Mobility-LLM-large, like many LLM-based approaches, lacks an explicit mechanism to model long-term dependencies effectively, leading to difficulties in capturing evolving user interests.

In contrast, our proposed TZPR models demonstrate robust adaptability across different sequence lengths. Unlike Mobility-LLM-large, TZPR maintains consistent performance gains as the trajectory length increases. This resilience is attributed to the model’s ability to dynamically integrate semantic, temporal, and spatial factors while leveraging its graph-based POI intent modeling. The incorporation of heterogeneous attention mechanisms enables TZPR to adjust its focus based on evolving user behaviors, preventing performance degradation on longer sequences.

Furthermore, the superior performance of TZPR across all trajectory lengths underscores its advantage in real-world POI recommendation scenarios, where users exhibit diverse mobility behaviors. For users with shorter histories, TZPR can extract meaningful patterns even from limited data, while for users with extensive check-in records, it effectively mitigates the challenges of interest drift and data saturation. These results highlight the limitations of traditional LLM-based POI recommenders and reaffirm the necessity of integrating domain-specific mobility modeling techniques, as exemplified by TZPR, to achieve more reliable and scalable POI recommendations.


% a. cloud-based recommender systems (privacy, high latency, long-tail issue)
% b. on-device recommender systems (federated & compressed & decentralized)
% limitation: low accuracy caused by two significant reasons:
% 1) cannot create user profile comprehensively
% 2) cannot retrieval large-scale items (many many items)
% 3）cold-start issue

% c. cloud-edge collaborative (need the help of cloud)
% challenges:
% 1. 在这样的情况下如何做隐私保护 - 建立用户画像
% 2. 任务分工 协作执行 - 复杂的推荐任务 - 复杂的推荐场景 可以介绍冷启动 这是why agent

% d. 可以引出 multi-agent

% e. 我们的work

% why agents?，可以描述agent的优势

% 需要一个智能助手

% agent优势（LLM优势）：利用大语言模型（LLM）驱动的 agent 能更好地理解用户语义、推理出用户的真实需求。
% agent优势 (可忽略)：agent 支持多轮对话、主动引导用户探索，形成更人性化的交互推荐。

% ！agent优势：agent 可以根据任务动态调整推荐策略，整合用户历史、目标和情境信息，生成定制化的推荐结果。
% ！agent优势：通过强化学习、自我优化机制、元学习等方式，agent 可实现持续学习和跨域迁移(冷启动，新领域)

% agent优势：多 agent 系统（multi-agent systems）支持角色分工，如一个负责抽象用户意图，另一个调用搜索工具，第三个进行精排等，模仿人类团队协作。
% agent优势：agent 可以根据任务动态调整推荐策略，整合用户历史、目标和情境信息，生成定制化的推荐结果。


% ➡️could-edge中需要重点关注两点/现有cloud-edge框架的问题：
% 1)edge-side: 需要提取与用户query相关的匿名化的关键信息 
% 2)could side: 要能充分理解edge side传来的少量信息，并进行large-scale retrieval

% ➡️LLM能够解决上述俩问题: 1) edge side: LLM is good task planner，这个很多工作的我们可以参考一下他们怎么讲的利用LLM做planning 2) cloud side: LLM powerful semantics understanding capability




% -----------------------------------------------------------
% 我现在的introduction思路是这样的，你看行不行：
% a. cloud-based recommender systems(privacy, high latency)

% b. on-device reommender systems (federated & compressed)
% low accuracy caused by:
% 1. cannot retrieval large-scale items (many many items)
% 2. cannot capture user preference comprehensively

% c. need the cloud-edge collaborative framework
% 主要描写challenges：
% 1 如何合作解决复杂的推荐任务 - 为了引出agent的planning 以及协作
% a. 根据用户的query以及实际情况动态调整推荐策略 - 一键式个性化推荐 推理用户需求
% b. 冷启动，新领域，在数据缺少的情况下如何进行推荐 - 为了引出LLM对自然语言的处理
% 2 在这样的情况下如何保护隐私

% d. multi-agent的兴起，描述multi-agent适合解决我们的问题

% e. 提出我们的framework，A Cloud-Edge Collaborative Multi-Agent
% Framework，如何解决上述挑战
% -----------------------------------------------------------
% 我感觉这个比之前好多了，但还是比较scattered，主要有几个点建议：

% b.2.能不能跟planning with agent结合，比如compressed的rec sys受限于参数量推理能力有限所以不能很好地规划任务，现在cannot capture user preference comprehensively还是太general 

% c.1.这样就可以自然引出agent planning，cloud-edge协作主要对应b.1 retrival这一device-side的缺点; 另外，冷启动这个问题要定义好，我理解这里应该是指利用llm的semantics能力解决item的冷启动问题，需要区别于user cold start

% c.2. privacy这个点我觉得属于device-side自带的优点，在前面介绍on-device rec sys的时候写就好了，写在challenge里有点混乱

% d. 基于上述challenge我们需要cloud-edge collaboration, 和llm->we propose a cloud-edge collaborative multi-agent framework。multi-agent不是最近才兴起的吧，之前做rl就有multi-agent的概念了，只是最近llm兴起，能有更智能的agent。



% limitations of LLM:
% 1. expensive to train and inference frequently
% 2. difficult to access real-time user behavior data
% why LLM + SRM?
% 因为互补



% collaborative training - planning 能力
% collaborative inference
% collaborative-decision request



% In the modern era, personalized recommender systems have become essential tools for assisting users in discovering relevant content and making informed decisions across various platforms. Traditional approaches, such as those based on graph neural networks (GNNs) and recurrent neural networks (RNNs), have demonstrated effectiveness in modeling behavioral patterns from historical interactions.


% 一定要强调agent的planning能力
% a. cloud-based recommender systems
% limitations: high latency, expensive, privacy,
% b. on-device recommender systems - low accuracy caused by:
% 1. 无法访问检索全量item库
% 2. 

% c. device-cloud recommendation
% 描述现有的 
% 缺少planning 能力，推荐范式固定，无法为不同的用户定制不同的推荐策略。
% 冷启动问题 - 忽略了用户语义理解能力，比如
% 云边协同效率低
% d. LLM-based multi-agent的火爆
% e. 受之启发，提出我们的模型


% SLM可以频繁地推理，实时行为，划分推荐内容


% a. cloud-based recommender systems (privacy, high latency, long-tail issue)
% b. on-device recommender systems (federated & compressed & decentralized)
% limitation: low accuracy caused by two significant reasons:
% 1) cannot create user profile comprehensively
% 2) cannot retrieval large-scale items (many many items)
% 3）cold-start issue

% c. cloud-edge collaborative (need the help of cloud)
% challenges:
% 1. 在这样的情况下如何做隐私保护 - 建立用户画像
% 2. 任务分工 协作执行 - 复杂的推荐任务 - 复杂的推荐场景 可以介绍冷启动 这是why agent

% d. 可以引出 multi-agent

% e. 我们的work


% 及时反馈推荐
% 音乐 新闻 短视频推荐（无数据）
% 延时反馈推荐
% movie POI
% \sr{I suggest to add one sentence here to introduce how RNNs/GNNs/LLMs-based methods are used in current cloud-device frameworks, or they are usually deployed on cloud/device solely.} 
% \sr{how RNNs and GNNs methods rely on cloud computing, not clear}
% \sr{i suggest to modify this para as: RNNs/GNNs/LLMs-based $\rightarrow$ current methods either depolyed on cloud (e.g.,call LLM API for linguistics info reasoning) or device (e.g., POI rec) $\rightarrow$ cloud only shortcomings (1 sentence). device only shortcomings (1 sentence) $\rightarrow$ so we need cloud-device collab}.

% In the modern era, personalized recommender systems have become essential tools for assisting users in discovering relevant content and making informed decisions across various platforms. Existing models such as those based on Recurrent Neural Networks (RNNs) \cite{xu2021long,duan2023long}, Graph Neural Networks (GNNs) \cite{he2020lightgcn,gao2022graph}, and more recently, Large Language Models (LLMs) \cite{lin2024data,acharya2023llm} have achieved great success in academia and industry. While effective, these methods rely heavily on cloud-based inference, which can introduce high latency and raise significant privacy concerns due to centralized data processing. In response, on-device recommender systems \cite{han2021deeprec,xia2022device,long2023model} have been explored to support low-latency, privacy-preserving inference by executing lightweight models locally on user devices. However, on-device approaches are fundamentally limited by the constrained computational and memory resources on user devices, which restrict model capacity and hinder their ability to perform large-scale retrieval or support sophisticated recommendation tasks. Consequently, on-device recommenders often exhibit relatively low accuracy compared to their cloud-based counterparts. % \sr{real-time computation that consider private data? locally observed signals is vague}

% Specifically, a candidate item set is first generated in the cloud using extensive item metadata and public user data. This set is then re-ranked on the device side using lightweight recommendation models (e.g., DIN \cite{zhou2018deep}), based on recent user behaviors and private user profiles. A representative model that adopts this cloud-device collaborative architecture is LSC4Rec \cite{lv2025collaboration}.
% The final recommendation outcome integrates signals from both perspectives, enabling the system to strike an effective balance between global generalization and local personalization

% \sr{i think the previous version emphasis the LSC4Rec too much. i modify a few sentences, plz check}.

%A representative example is LSC4Rec, which integrates a cloud-based large model with an on-device lightweight recommendation model (e.g., DIN \cite{zhou2018deep}). In this framework, the cloud module generates a candidate set and initial relevance scores based on globally available data. These are then transmitted to the user’s device, where the local model performs reranking using recent session behaviors and contextual information. The final recommendation result combines signals from both sides, allowing the system to achieve a balance between global generalization and local personalization.



% % 这一段需要改进,可能需要描述一系列方法，而不单单是这一个,或者说我应该简短地描述那些方法，再详细地描述下面这个方法，作为和我们方法的比较，这个需要斟酌一下。
% Motivated by the complementary advantages of cloud-based and on-device recommendation, recent work has investigated hybrid frameworks that integrate both paradigms \cite{lv2025collaboration,yao2022device,yao2021device}. As an advanced example, LSC4Rec integrates a cloud-based large language model with an on-device small recommendation model (e.g., DIN \cite{zhou2018deep}) to collaboratively perform recommendation. In this framework, the LLM on the cloud is responsible not only for generating the candidate set by retrieving semantically relevant items from the global item corpus, but also for providing an initial ranking of these candidates based on its understanding of user intent. The candidate set, along with the LLM-generated ranking scores, is then transmitted to the user's device, where the lightweight model conducts personalized reranking using recent session behaviors and local context. The final recommendation result is derived by combining the scores from both the LLM and the lightweight model, allowing the system to incorporate both global knowledge from the cloud and personalized signals from the device.

% \sr{Each user behaves differently under varying contextual conditions and demonstrates unique recommendation intents.}
% \sr{i think this example is a typical cold start problem. if cold start is the point, i suggest just use `cold start issue' as the subtitle.}
% \sr{examples r needed, e.g., the elder are readily to make wrong clicks}. 
% \sr{active state? should be more clear what is `state' here} and intent.
% \sr{existing methods}
% \sr{static collaboration architecture?}
% \sr{plz check}.%In some cases, unnecessary cloud involvement increases communication and computation overhead, while in others, insufficient cloud support hampers performance when local capabilities are limited. 
% Therefore, existing cloud-device collaboration systems struggle to balance efficiency and recommendation quality due to their inability to dynamically coordinate computational responsibilities based on user state, task complexity, or environmental conditions.
% %Without the ability to dynamically coordinate computational responsibilities based on user state, task complexity, or environmental conditions, current systems do not fully meet the demands of efficiency and recommendation quality.
% \sr{plz cehck. and i suggest to add more details of why interpretability especially important to cloud-device systems, compared to traditional rec}.
%The absence of transparent decision logic not only reduces user trust but also limits the system’s ability to support user feedback and refinement. 
%A framework that can trace and explain its planning and decision-making steps is essential for building trustable and user-aligned recommendation systems.

% Despite the promising architecture of existing cloud-device recommendation frameworks, two critical challenges remain unresolved:
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Lack of personalized strategy planning.} Existing cloud-device recommendation frameworks typically follow a fixed recommendation pipeline, lacking the ability to plan and adapt strategies according to task characteristics and behavioral sparsity. In practice, variability in user situation is commonly observed. For example, music or news platforms enable rapid feedback loops, where recommendations can be quickly refined based on immediate user responses, while book or movie recommendations involve delayed feedback and require more cautious, intent-aware decision-making. Similarly, active users with rich interaction histories may benefit from fine-grained personalization, whereas inactive users with limited behavioral signals demand more exploratory strategies. In this situation, applying a uniform recommendation process across such diverse scenarios can lead to degraded performance. 
%     \item \textbf{Inefficient Cloud-Device Collaboration.} Existing cloud-device recommendation frameworks often adopt a rigid division of labor, with the cloud typically responsible for candidate retrieval and the device handling local reranking. However, this fixed collaboration strategy often results in inefficient utilization of computational resources. For example, cloud-based retrieval may be unnecessarily invoked even when locally cached results or lightweight on-device heuristics would suffice, leading to increased server load and communication overhead. Conversely, when the device is resource-constrained or the user context demands more sophisticated modeling, insufficient cloud engagement may degrade recommendation quality. Without a mechanism to adaptively coordinate cloud and device resources based on task complexity, user state, or environmental factors, current systems do not fully meet the demands of efficiency and responsiveness.
%     \item \textbf{Inability to handle cold-start scenarios.} Current cloud-device recommendation systems rely heavily on historical user-item interactions to support personalized recommendations. However, in cold-start situations where there may be no usable behavioral data at all, these systems struggle to generate relevant results due to the absence of mechanisms for inferring user intent from limited context. As a result, recommendation quality degrades significantly, often leading to poor user experience and engagement.
% \end{itemize}
% These challenges call for a more flexible and intelligent cloud-device recommendation framework that can dynamically adapt recommendation strategies, efficiently coordinate resource usage, and effectively handle data-sparse scenarios such as cold-start.

% \sr{I think in this para, you should elaborate how LLMs/multi-agent system (MAS) benefit cloud-device collaboration systems in the aforementioned three challenges: 1) user heterogeneity, 2) more efficient collaboration 3) intepretability, respectively}

% This is achieved by utilizing the cloud-side LLM infers key 



% by analyzing contextual signals such as query specificity, behavior sparsity, and domain characteristics. 

% To achieve this, 

% By analyzing the user abstract—which encapsulates intent, behavioral summary, and domain information—the cloud-side LLM infers key contextual factors such as query specificity, interaction sparsity, and feedback dynamics. 

% It then synthesizes a personalized recommendation strategy that determines how to allocate modeling and inference tasks across cloud and device in a manner tailored to the user’s current needs. 

% This strategy-guided design allows CDARA to move beyond fixed recommendation pipelines, enabling flexible adaptation to diverse scenarios while improving both personalization effectiveness and resource coordination. 



% Based on this analysis, it flexibly allocates tasks between the cloud and the device, enhancing both personalization effectiveness and cloud-device collaboration efficiency. 



% In addition, CDARA naturally supports interpretable outputs since each step in the pipeline is planned and executed explicitly, with traceable reasoning paths and adaptive decisions. Our main contributions are summarized as follows:



% Additionally, CDARA also enhances transparency and explainability in the recommendation process. Since each step in the pipeline is planned and executed explicitly, with traceable reasoning paths and adaptive decisions, CDARA naturally supports interpretable outputs. 





% Our main contributions are summarized as follows:


% Specifically, the recommendation process begins on the device, where the lightweight SLM generates a user abstract that summarizes intent and behavioral patterns in a privacy-preserving manner. This abstract is then transmitted to the cloud, where the powerful LLM-based strategy planner analyzes the abstract along with domain information to formulate a personalized recommendation plan, which governs the allocation of modeling and inference tasks between cloud and device. For example, in domains with rapid feedback cycles such as music or news, the strategy may emphasize short-term signals and lightweight modeling. In contrast, domains like movies or travel may favor more intent-focused strategies that rely on semantic reasoning. Based on the generated plan, the cloud agent performs semantic user modeling and coarse candidate retrieval, returning a personalized candidate set to the device. The device agent then selectively conducts structured modeling using local interaction history and completes final ranking by fusing semantic and structured representations. The device agent then selectively conducts structured modeling using local interaction history and completes final ranking by fusing semantic and structured representations, as well as generating user-facing explanations based on the planned strategy and observed user signals. This cloud-device collaboration framework, guided by strategy planning, allows CDARA to flexibly adapt to varying user contexts and optimize resource usage in a secure and interpretable manner. 

% \begin{itemize}[leftmargin=*]
%     \item We propose CDARA, a novel cloud-device recommendation framework based on a multi-agent architecture. CDARA leverages the complementary strengths of a cloud-based large language model (LLM) and an on-device small language model (SLM) to collaboratively perform recommendation tasks. This architecture allows the system to better interpret user intent, capture both long-term and contextual preferences, and deliver high-quality recommendations while preserving privacy and ensuring responsiveness.

%     \item We introduce a strategy planning mechanism that dynamically generates personalized recommendation plans. By analyzing the user’s abstracted intent and domain characteristics, the cloud-side LLM determines how to allocate modeling and inference tasks across cloud and device. This enables both more accurate personalization and efficient cloud-device collaboration, reducing unnecessary computation and transmission.

%     \item We enhance interpretability by enabling explicit, step-by-step reasoning throughout the recommendation pipeline. CDARA’s design allows the system to trace and verbalize the rationale behind specific modeling choices and recommendation results, thereby providing users and developers with a transparent and trustworthy experience.

%     \item We conduct extensive experiments on multiple benchmark datasets. Results demonstrate that CDARA outperforms strong baselines in both accuracy and efficiency, validating its effectiveness under diverse user behaviors and recommendation domains.
% \end{itemize}





% \section{Introduction}
% In the modern era, personalized recommender systems have become essential tools for assisting users in discovering relevant content and making informed decisions across various platforms. Traditional approaches, such as those based on graph neural networks (GNNs) and recurrent neural networks (RNNs), have demonstrated effectiveness in modeling behavioral patterns from historical interactions. However, these methods often rely on extensive feature engineering, struggle with generalization in cold-start scenarios, and lack the capacity for semantic reasoning\sr{here you propose 3 shortcomings of traditional rec: 1) extensive feature engineering 2) cold-start 3) lack of semantic reasoning}. The recent advent of large language models (LLMs) has introduced a new paradigm in recommendation. With their strong generalization ability, deep semantic understanding, and powerful zero-shot reasoning capabilities, LLMs can infer user preferences and generate rich representations for users and items directly from unstructured inputs (e.g., natural language queries). This enables more flexible and context-aware recommendation, particularly in cold-start settings where traditional models fall short\sr{i suggest just briefly mention that the advent of LLMs can address the above three shortcomings.}.

% \sr{then in this paragraph illustrate in details how LLM address the three shortcomings with literature}Building upon this progress, recent works have explored the use of LLM-based agents for recommendation tasks. By leveraging their strong semantic understanding, planning capabilities, and decision-making skills, these agents enable more nuanced, context-aware, and personalized recommendations. Specifically, \cite{wang2023c, zhang2024generative, zhang2024agentcf} focus on employing LLM-based agents for simulating user behaviors, providing insights into user preferences but falling short of integration into recommender systems. In contrast, \cite{huang2023recommender,wang2023recmind} attempt to construct recommender models driven by a single LLM-based agent, which is augmented with planning, memory mechanisms, and auxiliary tools (e.g., search engine). In addition, some studies \cite{shu2023rah,wang2024macrec} take a step further by enabling multiple agents to cooperate or compete with one another, thereby mimicking human workflows and collaboratively accomplishing recommendation tasks.


% While LLM-based agents have opened new possibilities for personalized recommendation, several critical limitations hinder their practical deployment\sr{are there any connections between the following limitations and the aforementioned shortcomings?}:
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Privacy and Latency Concerns Stemming from Cloud Reliance}. Existing approaches typically rely on executing large language models on cloud servers, which introduces two major issues. First, uploading sensitive user data to external servers raises significant privacy concerns, particularly in domains where user behaviors, preferences, or locations must be carefully protected. Second, in this cloud-centered paradigm, user devices merely act as terminals for transmitting user data and displaying server-generated recommendations, making the recommendation process heavily dependent on server capacity and internet connectivity. This reliance not only increases latency but also undermines system resilience, particularly in resource-constrained or offline environments.\sr{privacy and latency are both important, i suggest to split them into two limitations}
%     \item \textbf{Limited Incorporation of Structured Behavioral Data}. While LLM-based agents demonstrate strong capabilities in interpreting user queries expressed in natural language, they primarily focus on semantic reasoning over unstructured text and pay limited attention to structured behavioral interaction histories. However, in personalized recommendation, historical user-item interactions provide crucial signals that cannot be fully captured through semantic interpretation alone. For example, a user with a long-standing preference for science fiction novels might submit a vague query like "recommend me something exciting," and an LLM, reasoning purely from surface semantics, may suggest an action movie or a thriller, overlooking the deeper behavioral patterns encoded in the user's historical interactions. This gap arises because standard LLM architectures are pretrained predominantly on natural language corpora and lack native mechanisms to integrate structured, sequential behavioral data. Consequently, recommendations generated solely by LLM agents may appear contextually plausible but fail to align with users’ long-term interests, leading to suboptimal personalization outcomes.
%     \item \textbf{Inefficient Task Planning and Ineffective Multi-Agent Collaboration}. Many existing LLM-based recommendation agents treat the recommendation process as a monolithic, single-shot operation, relying on LLMs to directly generate recommendations or retrieve items based on textual matching. This approach lacks modular task decomposition, making it difficult to support complex recommendation workflows that involve distinct stages such as intent understanding, user modeling, coarse candidate retrieval, fine ranking, and explanation generation. As a result, subtasks that could otherwise benefit from specialization and parallel execution are often processed sequentially, leading to high inference latency. Furthermore, current systems typically assume a small, predefined candidate pool for retrieval, which is impractical for real-world recommendation scenarios. Effective recommendation demands the ability to operate over millions of candidate items and rapidly identify relevant subsets, a requirement that existing LLM-based approaches fail to meet at scale.
% \end{itemize}

% To address the challenges of privacy, latency, scalability, and automation in personalized recommendation, we propose a multi-agent framework that enables secure, efficient, and fully automated recommendation generation. The framework incorporates three specialized agents that collaborate to complete the end-to-end recommendation pipeline. A device-side Coordinator Agent interprets the user query, retrieves relevant profile, context, and interaction signals, and constructs a structured, privacy-preserving prompt. This abstracted prompt is sent to the cloud-side Retrieval Agent, which uses a large language model to generate a semantic user embedding and retrieve a coarse candidate set from the relevant item domain. In parallel, the device-side Ranking Agent computes a structured behavioral embedding using lightweight local models. These two embeddings are fused to re-rank the candidates and generate a personalized Top-$K$ list, followed by optional on-device explanation generation to improve transparency and trust. To further improve efficiency, item embeddings are initialized through LLM-based textual encoding and organized into semantic or location-aware groups, enabling scalable coarse retrieval. By combining modular task decomposition, parallel processing, and privacy-preserving agent collaboration, our framework achieves high-quality recommendations with low latency and minimal user effort. Our main contributions are summarized as follows:

% \begin{itemize}[leftmargin=*]
%     \item We propose a multi-agent recommendation framework that supports secure, low-latency, and fully automated recommendation generation. The system introduces three collaborative agents—Coordinator, Retrieval, and Ranking—that divide the end-to-end recommendation workflow into modular subtasks. Each agent is responsible for a specific aspect of the pipeline, enabling flexible orchestration while ensuring that sensitive user data is processed exclusively on the device.

%     \item We design a dual-embedding personalization strategy that captures both user intent and behavioral patterns. The semantic embedding is generated from abstracted user descriptions via a cloud-based large language model, while the structured embedding is derived from the user's interaction history using lightweight on-device models. These two representations are fused to support fine-grained ranking tailored to both short-term and long-term preferences.

%     \item To improve system efficiency and scalability, we implement parallel execution of semantic and behavioral modeling, which operate independently on different inputs. In addition, we construct item embeddings using LLM-based textual encoding and organize them into domain-specific or group-based clusters. This design significantly accelerates coarse candidate retrieval across large item pools.

%     \item We conduct extensive experiments on multiple real-world recommendation datasets. Results show that our framework outperforms strong baselines in terms of recommendation accuracy, inference latency, candidate scalability, and privacy protection, demonstrating the effectiveness and practicality of our design.
% \end{itemize}
% \sr{}

Personalized recommender systems play a critical role in helping users discover relevant content across digital platforms. Traditional models such as graph neural networks (GNNs) and recurrent neural networks (RNNs) are effective in modeling historical behaviors, but they often struggle with cold-start scenarios and lack semantic reasoning capabilities. Recent advances in large language models (LLMs) have led to the emergence of LLM-based agents for recommendation, offering new opportunities through their strong generalization and language understanding abilities. However, existing LLM-based recommendation agents face three critical limitations: (1) privacy concerns arising from reliance on cloud-based inference, (2) limited integration of structured behavioral data, and (3) inefficient task planning due to the lack of modular multi-agent collaboration. To address these challenges, we propose a cloud-edge collaborative multi-agent recommendation framework (CCMPR). The framework introduces three specialized agents that coordinate to complete modular subtasks across device and cloud environments. Device-side agents handle user intent classification, behavior modeling, and prompt construction using only local data, while the cloud-side agent leverages an LLM to perform semantic user modeling and coarse candidate retrieval. The resulting embeddings are fused on-device to generate a personalized Top-$K$ recommendation list, optionally accompanied by natural language explanations. Extensive experiments on real-world datasets demonstrate that CCMPR outperforms strong baselines in terms of recommendation accuracy, scalability, latency, and privacy protection, validating its effectiveness and practicality.

% MF+markov chains
% gnn
% rnn
% attention
% LLM



% Sequential recommendation algorithms model users’ behavior sequences and predict their next actions. They have been widely
% applied in scenarios such as e-commerce, short video recommendations, education, and healthcare. 

% Classic recommendation models
% such as Caser [41], GRU4Rec [12], DIN [64], and SASRec [15] are
% still commonly used today. In recent years, many studies have focused on different aspects of sequential recommendation, such as
% personalization [32–34, 38], multimodality [14, 51, 54, 55], privacy
% protection [20], user feedback [9, 56], cross-domain [27, 63], cold
% start [4, 28], long-tail [59], session-based [37], debias [3], structure
% learning [7], disentanglement [5], LLM-based [2, 58], generativebased [23, 60], fairness [47], etc. Although Sequential Recommendation Models (SRMs) require fewer hardware resources and are
% easier to deploy on devices, they have limitations in feature extraction and generalization capabilities. These studies, however, have
% not addressed the deployment of SRMs on devices or the associated
% limitations




% Sequential recommendation models the evolving interests of users based on historical interactions~\cite{quadrana2018sequence,fang2019deep}. Traditional methods employ recurrent neural networks (GRU4Rec~\cite{hidasi2015session}), convolutional networks (Caser~\cite{tang2018personalized}), or transformer-based self-attention mechanisms (SASRec~\cite{kang2018self}) to capture sequential dynamics. 



% Recently, Large Language Models (LLMs) have shown strong potential by reformulating sequential recommendation as generative tasks, benefiting from rich semantic context~\cite{raffel2020exploring,bao2023tallrec}. For instance, P5~\cite{raffel2020exploring} treats recommendation subtasks as text-to-text generation, and TALLRec~\cite{bao2023tallrec} further enhances performance by instruction tuning. 

% Similarly, RecFormer~\cite{li2022recformer} treats recommendation purely as a language modeling task, directly modeling item sequences as textual input to leverage rich semantic information. MoRec~\cite{hou2023morec} introduces a mixture-of-experts approach for LLM-based recommendation, routing inputs through specialized recommendation and language experts. 

% ChatRec~\cite{gao2023chat} explores conversational recommendation through natural language interactions, while InstructRec~\cite{zhang2023instructrec} leverages instruction tuning to align language model capabilities with recommendation objectives. 

% However, purely generative LLM approaches often face limitations in explicitly leveraging relevant external context, potentially hindering their performance in sparse or ambiguous recommendation scenarios~\cite{hou2023morec,hou2024large}.

% This multi-agent design brings greater flexibility, interpretability, and adaptability to complex recommendation scenarios.


% More recently, large language models (LLMs) have been applied to sequential recommendation due to their powerful generative and reasoning capabilities. Works such as P5~\cite{geng2022recommendation}, LLM4Rec~\cite{zhao2024llm}, and ReLLLa~\cite{yu2024retrieval} reformulate recommendation tasks as natural language problems, enabling zero-shot and few-shot prediction by prompting pretrained LLMs with user histories and item metadata. While effective, these methods often rely on cloud-based inference, limiting real-time personalization and raising privacy concerns.

% To address these challenges, recent efforts explore LLM-based agent frameworks for sequential recommendation. For example, MACRec~\cite{wang2024macrec} and AdaRAG~\cite{wu2024adarag} adopt multi-agent designs, where specialized LLM agents handle retrieval, ranking, and reasoning tasks in a modular and interpretable manner. These approaches show promising performance and flexibility but often lack adaptation to device constraints or dynamic user needs.

Sequential recommendation aims to model the evolving preferences of users based on their historical interactions. Early methods primarily relied on matrix factorization~\cite{mehta2017review} and Markov chains~\cite{rendle2010factorizing}, which respectively modeled users’ general preferences and short-term item transitions. However, these methods were limited in capturing complex dependencies and evolving user intent over longer sequences. To capture sequential dependencies in user behavior, recurrent neural network-based methods and their variants \cite{hidasi2015session,xu2021long,cui2018mv} have been proposed to model user interaction histories as ordered sequences. These approaches effectively learn short-term and local patterns by updating hidden states over time. Graph-based methods \cite{liu2024selfgnn,chang2021sequential,zhang2022dynamic} offer an alternative paradigm for sequential modeling by representing item transitions as graphs derived from user sessions. These approaches leverage graph neural networks to capture complex dependencies and high-order relationships among items, enabling richer contextual reasoning and improved representation of sequential behaviors. To enhance sequential modeling, attention mechanisms \cite{kang2018self,li2020time} have been introduced as flexible components that can be integrated into RNNs, GNNs, or used independently. In particular, self-attention effectively captures global dependencies in user behavior sequences, enabling parallel and context-aware recommendation.

% Specifically

% In more realistic recommendation scenarios, effective collaboration between device-side and cloud-side models is often necessary. 


% Early frameworks such as MetaController and DCCL introduced dynamic collaboration strategies that allow the system to switch between cloud and device recommenders based on user behavior patterns. 


% DUET and IntellectReq focused on enhancing the generalization ability of device models by enabling the cloud to generate personalized parameters or determine communication needs using uncertainty estimation. 


% Finally, LSC4Rec proposed a collaborative framework that integrates a cloud-based LLM with an on-device SRM, supporting joint training and inference to leverage the strengths of both models across cloud and edge environments.

% This paradigm improves scalability and efficiency, but its effectiveness depends on how well the cloud and device are coordinated.



% To overcome the limitations of purely on-device recommendation, recent research has explored cloud-device collaborative frameworks that split the recommendation process across the cloud and local device. In this setting, the cloud model typically handles computationally intensive tasks such as candidate generation, semantic retrieval, or global user modeling, while the device-side model focuses on real-time personalization using local context, such as recent interactions or behavioral signals.

% This collaborative architecture aims to combine the scalability and modeling capacity of cloud-based systems with the responsiveness and privacy benefits of on-device inference. Representative works adopt a two-stage pipeline: the cloud component generates a candidate set and preliminary scores based on global knowledge, and the device-side model performs reranking or filtering based on local user signals. Such designs have shown promise in reducing inference latency while preserving recommendation quality.

% However, most existing frameworks rely on static collaboration patterns, assigning fixed roles to the cloud and device regardless of the user state, query specificity, or task complexity. This limits their adaptability and may lead to suboptimal resource allocation or degraded personalization in dynamic scenarios. To address this, more flexible and intelligent coordination mechanisms are needed to tailor cloud-device collaboration to individual user contexts.

% Done
% On-device frameworks effectively address many limitations of cloud-based learning in POI recommendations. Federated learning \cite{2021PREFER}, a key approach in this context, aggregates locally trained models and shares a unified model with users. However, this can result in the long-tail problem, where less active users get subpar recommendations. Some federated POI recommenders \cite{2020xw,2021rao} tackle this by grouping users with similar interests, and decentralized systems \cite{long2023decentralized,long2023model} allow nearby devices to collaborate, enhancing personalization. Despite this, these methods demand extensive device engagement and intra-device communication, raising concerns about privacy and Transferability. An alternative approach \cite{2020Next} is using pre-trained, compressed models on devices with anonymized data for privacy, but this compromises accuracy due to the lack of personalized data and limited model adaptability. Some systems \cite{mairittha2020improving,yan2022device} try to fine-tune with local data, yet they underperform compared to centralized systems. Although this method can quickly adapt to new users, it compromises recommendation quality and struggles to adjust to new regions. Our work introduces a diffusion model-based system, deploying a well-trained model to users for local fine-tuning and achieving high-quality recommendations.

% \begin{table*}[t]
% \centering
% \caption{Performance comparison across datasets and methods}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccccccccccccc}
% \toprule
% \textbf{Method} & \multicolumn{4}{c}{\textbf{Movie}} & \multicolumn{4}{c}{\textbf{Music}} & \multicolumn{4}{c}{\textbf{Sports}} & \multicolumn{4}{c}{\textbf{POI}} \\
% & HR@5 & NDCG@5 & HR@10 & NDCG@10 & HR@5 & NDCG@5 & HR@10 & NDCG@10 & HR@5 & NDCG@5 & HR@10 & NDCG@10 & HR@5 & NDCG@5 & HR@10 & NDCG@10 \\
% \midrule
% \multicolumn{17}{c}{\textit{Cloud-side Inference}} \\
% GRU4Rec & 0.0111 & 0.0069 & 0.0199 & 0.0099 & 0.0105 & 0.0061 & 0.0185 & 0.0086 & 0.0089 & 0.0053 & 0.0162 & 0.0077 & 0.2536 & 0.1876 & 0.3615 & 0.2177 \\
% SASRec & 0.0143 & 0.0085 & 0.0256 & 0.0131 & 0.0132 & 0.0079 & 0.0233 & 0.0108 & 0.0101 & 0.0067 & 0.0191 & 0.0094 & 0.2614 & 0.1967 & 0.3741 & 0.2293 \\
% SR-GNN & 0.0181 & 0.0111 & 0.0305 & 0.0159 & 0.0156 & 0.0092 & 0.0263 & 0.0123 & 0.0118 & 0.0072 & 0.0207 & 0.0106 & 0.2955 & 0.2150 & 0.3976 & 0.2485 \\
% RARec & 0.0235 & 0.0166 & 0.0394 & 0.0240 & 0.0233 & 0.0155 & 0.0388 & 0.0229 & 0.0128 & 0.0090 & 0.0230 & 0.0125 & 0.3220 & 0.2328 & 0.4489 & 0.2669 \\
% \midrule
% \multicolumn{17}{c}{\textit{Device-side Inference}} \\
% LLRec & 0.0099 & 0.0059 & 0.0177 & 0.0085 & 0.0091 & 0.0053 & 0.0163 & 0.0076 & 0.0079 & 0.0046 & 0.0145 & 0.0066 & 0.2216 & 0.1613 & 0.3073 & 0.1950 \\
% PREFER & 0.0103 & 0.0065 & 0.0183 & 0.0092 & 0.0098 & 0.0058 & 0.0174 & 0.0081 & 0.0083 & 0.0050 & 0.0151 & 0.0070 & 0.2392 & 0.1768 & 0.3392 & 0.1974 \\
% \midrule
% \multicolumn{17}{c}{\textit{Cloud-device Collaborative Inference}} \\
% DCCL & 0.0145 & 0.0086 & 0.0264 & 0.0133 & 0.0134 & 0.0081 & 0.0239 & 0.0111 & 0.0103 & 0.0068 & 0.0193 & 0.0095 & 0.2621 & 0.2019 & 0.3796 & 0.2360 \\
% DUET & 0.0172 & 0.0107 & 0.0285 & 0.0149 & 0.0148 & 0.0087 & 0.0252 & 0.0115 & 0.0109 & 0.0069 & 0.0195 & 0.0102 & 0.2872 & 0.2094 & 0.3908 & 0.2422 \\
% LSC4Rec & 0.0242 & 0.0170 & 0.0401 & 0.0253 & 0.0242 & 0.0164 & 0.0396 & 0.0236 & 0.0133 & 0.0094 & 0.0236 & 0.0130 & 0.3290 & 0.2387 & 0.4607 & 0.2799 \\
% Our Method & 0.0259 & 0.0182 & 0.0423 & 0.0271 & 0.0256 & 0.0178 & 0.0426 & 0.0250 & 0.0176 & 0.0121 & 0.0275 & 0.0174 & 0.3589 & 0.2576 & 0.4845 & 0.3046 \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:RA}
% \end{table*}

% \begin{table}[t]
% \centering
% \caption{Comparison of HR@10 and inference time (IT in milliseconds) across datasets and strategies}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{l|cc|cc|cc|cc}
% \toprule
% \textbf{Method} & \multicolumn{2}{c|}{\textbf{Movie}} & \multicolumn{2}{c|}{\textbf{Music}} & \multicolumn{2}{c|}{\textbf{Sports}} & \multicolumn{2}{c}{\textbf{POI}} \\
% & HR@10 & IT & HR@10 & IT & HR@10 & IT & HR@10 & IT \\
% \midrule
% LSC4Rec & 0.0401 & 677.16 & 0.0364 & 1500.72 & 0.0236 & 531.32 & 0.4607 & 325.05 \\
% CDARA   & \textbf{0.0423} & \textbf{88.95}  & \textbf{0.0398} & \textbf{93.41}   & \textbf{0.0304} & \textbf{70.48}   & \textbf{0.4845} & \textbf{82.35} \\
% \midrule
% $v_1$   & 0.0415 & 89.16  & 0.0379 & 95.51   & 0.0239 & 70.76   & 0.4597 & 44.29 \\
% $v_2$   & 0.0409 & 91.03  & 0.0337 & 94.89   & 0.0221 & 71.96   & 0.4471 & 44.01 \\
% $v_3$   & 0.0358 & 91.17  & 0.0362 & 93.80   & 0.0235 & 71.07   & 0.4512 & 44.08 \\
% $v_4$   & 0.0338 & 28.82  & 0.0281 & 31.67   & 0.0207 & 24.30   & 0.4717 & 14.27 \\
% $v_5$   & 0.0412 & 91.81  & 0.0385 & 95.93   & 0.0243 & 72.23   & 0.4482 & 42.96 \\
% $v_6$   & 0.0393 & 89.33  & 0.0315 & 97.06   & 0.0211 & 73.06   & 0.4172 & 42.93 \\
% $v_7$   & 0.0377 & 89.76  & 0.0361 & 95.06   & 0.0232 & 71.16   & 0.4711 & 43.06 \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:RQ2}
% \end{table}


% 不同的模型在不同的领域有着不同的表现，需要strategy


% Table~\ref{tab:main_results} reports the top-$K$ recommendation accuracy across four domains, where CDARA consistently achieves the best performance. This clearly demonstrates the superiority of our collaborative framework, which dynamically allocates tasks between cloud and device based on user context. CDARA not only leverages the powerful semantic reasoning of LLMs but also adapts to real-time device-side signals via structured modeling, achieving precise and timely personalization.

% Furthermore, our results reveal interesting cross-domain insights. In domains with high interaction sparsity (e.g., Sport), the advantage of CDARA is more pronounced, suggesting that dynamic strategy adjustment is particularly effective in addressing data scarcity. Meanwhile, in dense domains (e.g., Music), models like TGCL4SR and TransRec also perform well, but still fall short of CDARA due to their lack of adaptive and context-aware task assignment.




% Among cloud-side inference methods, TGCL4SR shows relatively strong performance due to its integration of a temporal-aware item transition graph and a Transformer encoder, which effectively captures both evolving user intents and global item relations. In contrast, models relying solely on sequential modeling (e.g., GRU4Rec and SASRec) or static neighborhood aggregation (e.g., LightGCN) exhibit inferior performance due to limited adaptability and lack of temporal granularity. RARec and TransRec, as LLM-based frameworks, also yield competitive results by bridging language and recommendation spaces via learned ID-token alignments. However, their reliance on large-scale LLM inference leads to latency and scalability issues, especially in resource-constrained environments.




% Table~\ref{tab:main_results} reports the top-$K$ recommendation accuracy across four domains, where CDARA consistently achieves the best performance. This clearly demonstrates the superiority of our collaborative framework, which dynamically allocates tasks between cloud and device based on user context. CDARA not only leverages the powerful semantic reasoning of LLMs but also adapts to real-time device-side signals via structured modeling, achieving precise and timely personalization.



% In the device-side inference group, models like LLRec, PREFER, and DCCL suffer noticeable performance degradation. This can be attributed to the limited modeling capacity and computational constraints on edge devices, which restrict the use of advanced architectures like transformers or LLMs. Though DCCL introduces personalization via MetaPatch, its inability to utilize rich semantic priors from cloud-based models hinders its recommendation quality.

% Collaborative frameworks provide a middle ground, balancing accuracy and efficiency. DUET achieves fast adaptation by forwarding cloud-side parameters, but lacks fine-grained personalization. LSC4Rec, on the other hand, employs both LLMs and structured models across device and cloud, outperforming most baselines. However, its static pipeline and absence of adaptive user strategy planning limit its further gains. CDARA outperforms LSC4Rec by introducing a context-aware strategy planner that tailors the collaboration path for each user scenario—e.g., allocating more modeling to the cloud for cold-start users or prioritizing device-side inference for high-frequency users—thus realizing fine-grained personalization and efficient coordination.

% Furthermore, our results reveal interesting cross-domain insights. In domains with high interaction sparsity (e.g., Sport), the advantage of CDARA is more pronounced, suggesting that dynamic strategy adjustment is particularly effective in addressing data scarcity. Meanwhile, in dense domains (e.g., Music), models like TGCL4SR and TransRec also perform well, but still fall short of CDARA due to their lack of adaptive and context-aware task assignment.


% The results show that CDARA significantly outperforms all baselines in inference speed, with a per-sample latency under 100 ms across all domains. In contrast, LLM-based methods (RARec and TransRec) suffer from high inference costs due to autoregressive generation and complex token grounding, especially in larger domains like Music. LSC4Rec, while incorporating some collaborative inference strategies, still incurs substantial overhead due to its static pipeline and limited optimization for device-side execution.

% In contrast, CDARA achieves superior efficiency by offloading simple tasks to the device, minimizing reliance on heavy cloud inference. Its context-aware planner dynamically adjusts the inference path per user, reducing unnecessary computation and communication. This design allows CDARA to maintain low latency without sacrificing accuracy, making it highly suitable for real-world, resource-constrained recommendation settings.

% To enable effective semantic reasoning and personalized planning on the cloud while preserving user privacy, we design a lightweight abstraction mechanism on the device. Instead of directly uploading raw user data such as queries or interaction logs, the device agent summarizes the user’s current state into a compact natural language form. This allows the cloud agent to access essential signals for downstream planning without requiring access to sensitive or fine-grained user behavior. This abstraction serves as a privacy-aware bridge between device-collected context and cloud-side semantic decision-making.
% % user intent, behavioral sparsity, and short-term interest shifts

% Upon receiving a recommendation query $q_u$, the device-side agent utilizes a light-weight SLM $\Theta_s$ to generate a natural language summary referred to as the personalized user abstract $a_u$, which consists of two parts. The first is a sanitized query, obtained by rephrasing the original user query to remove sensitive or overly specific personal information while retaining its core intent. The second is a behavioral summary built from the user's interaction history, which reflects user-level behavioral signal including interaction sparsity, long-term preference trends, and recent short-term interests. The abstract is generated using a prompt-driven interface, where the SLM receives an instruction prompt that explicitly guides it to produce the two-part output:
% \begin{promptbox}  
% \textbf{Prompt for Abstract Generation:}\\
% \textit{\textcolor{purple}{ Given the current user's query and interaction history, generate a two-part abstract: (1) a sanitized query that preserves intent while removing sensitive or overly specific content, and (2) a behavioral summary describing interaction sparsity and preference patterns without referencing specific items.}}\\
% \\
% Query: \textcolor{teal}{$q_u$}\\
% Interaction History: \textcolor{teal}{$\{(\text{text}(i),t_i) \mid i \in \mathcal{X}_u\}$}\\
% \\
% \textbf{Output Example:} \\ 
% \textbf{Query}\\
% The user is looking for some comfortable sport shoes.\\
% \textbf{Behavior Summary}\\ 
% The user has 3 sports-related interactions in total, all of which occurred within the past week. There is no significant long-term activity, resulting in the absence of identifiable long-term preferences. In the short term, the user shows a clear interest in badminton-related items.
% \end{promptbox}
% \noindent Here, $\text{text}(i)$ and $t_i$ are the natural language description (e.g., title and tags) and the interacted timestamp for the item $i$.

% \textbf{Interpretable Planning via Prompting.} To realize this reasoning process, CDARA employs a prompt-driven interface that instructs the cloud agent to analyze the abstract and return a structured plan. The prompt includes a breakdown of each module’s decision criteria and enforces a unified output format for ease of parsing and downstream execution.



% To operationalize the planning process, we distill the above analyses and constraints into a carefully designed prompt. This prompt guides the cloud-based LLM to generate an adaptive recommendation strategy by specifying the execution decisions for each module. The prompt clearly defines the task, provides necessary context from the user abstract, and enforces a structured output format to ensure consistency, interpretability, and ease of downstream parsing:
% We translate the above design considerations into a prompt-driven interface that enables the cloud-based LLM to generate adaptive, per-user recommendation strategies. This prompt explicitly defines the planning task, supplies the user abstract as input, and incorporates execution constraints in a structured output format. In doing so, we ensure that the generated strategies are both personalized and system-efficient.




% In cloud-device collaborative recommendation framework, blindly executing a fixed pipeline for every user limits both personalization and system efficiency. To address this, we introduce a strategy planning module that dynamically determines how the recommendation task should be routed and executed based on the user’s current query, behavioral summary, and domain characteristics. To enable flexible and context-aware recommendation, CDARA performs strategy planning on the cloud using a powerful LLM. Unlike the lightweight SLM on the device, the LLM can better interpret nuanced user intent, assess task complexity, and coordinate system-wide execution. To preserve user privacy, the planning process relies solely on the abstract generated by the device without exposing raw user data. The integration of explicit strategy planning enhances the overall performance of our cloud-device recommendation framework in two key ways. One one hand, it enables more accurate interpretation of user needs by dynamically adapting the recommendation process to user states. On the other hand, it reduces both computational load and communication overhead not only by selectively activating modules, but also by partially executing components when full processing is unnecessary. 

% Apart from Abstract Generation and Strategy Planning, our proposed CDARA comprises four core components including Semantic User Modeling, Candidate Retrieval, Structured User Modeling, and Final Ranking with Explanation Generation. The generated personalized plan determines how each of these components should be adaptively executed. In what follows, we first examine how user-specific states influence the behavior of these modules. We then integrate these factors into a structured prompt, enabling the LLM to generate interpretable and reliable execution plans.

% \begin{itemize}[leftmargin=*]
%     \item\textbf{Semantic User Modeling.} This module constructs a semantic user representation based on the user abstract, which includes both the sanitized query and the behavioral summary. The informativeness of each part plays a critical role in determining the quality of the resulting semantic embedding. For instance, greater emphasis should be placed on the query if it clearly expresses the user's intent. In contrast, the behavioral summary should carry more weight when the user has a rich interaction history, particularly if that history reflects recent interests. Therefore, the LLM is expected to first assess the informativeness of each component and determine their relative contributions accordingly, which serves as the basis for generating a high-quality semantic embedding. 
%     % The recommended strategy format for this module is: Assign 40\% weight to the query and 60\% weight to the behavioral summary to build the semantic user embedding.
    
%     \item\textbf{Candidate Retrieval.} This module is responsible for generating a relevant and computationally efficient candidate set from the large-scale item corpus. Computing similarities for every item even within the related domain is prohibitively expensive, so CDARA adopts a two-step approach. First, it selects a set of tags that are highly relevant to the user based on their intent and behavioral signals. Then, it retrieves items only from those selected tag groups. Using the same retrieval strategy for every user, such as a fixed number of tags or a fixed candidate pool size, can be inefficient and inaccurate. A rigid strategy may fail to capture user-specific needs or lead to wasted computation and communication due to irrelevant or excessive candidates. 

%     % we find the fact that.
%     To ensure both effectiveness and efficiency, we introduce adaptive tag and candidate levels. The number of tags and the total size of the candidate set are determined dynamically based on user-specific signals. For example, if the query and behavioral summary clearly express the user’s intent, fewer tags and a more compact candidate set may be sufficient. In contrast, when the intent is ambiguous or behavioral data is sparse, broader retrieval helps maintain coverage. These decisions are also guided by the characteristics of the recommendation domain. For instance, domains such as news or music may require more tags and a larger candidate pool to capture freshness and diversity, while more static domains like movies may benefit from smaller, focused selections.

%     CDARA leverages a cloud-based LLM to analyze the clarity of the query, the quality and recency of behavioral signals, and the semantic demands of the domain. Based on this analysis, the LLM decides the appropriate number of tags and the size of the candidate set. To ensure the strategy remains interpretable and bounded, we constrain the LLM’s output to predefined options: tag counts from \{3, 5, 10, 20\} and candidate sizes from \{500, 1000, 2000, 5000\}. The LLM also assigns a weight to each selected tag group to determine how many candidates should be retrieved from each.
%     % A representative output may look like:
%     % Retrieve 500 candidates from the badminton group, 300 from the footwear group, and 200 from the activewear group.

%     \item\textbf{Structured User Modeling.} This module generates a structured user embedding based on the user's sequential interaction history. Before proceeding, the LLM first evaluates whether structured modeling is necessary by analyzing the quantity and recency of past interactions. If the history is too sparse or outdated, the system may skip this step to conserve computational resources. When modeling is deemed beneficial, the system selects an appropriate encoder from a predefined set, which currently includes SR-GNN and SASRec. SASRec captures sequential dependencies through self-attention and is well-suited for modeling users with clear interaction patterns. In contrast, SR-GNN leverages a session-based graph structure to model complex item transitions, making it effective when the interaction sequence exhibits non-linear or contextual dependencies.
%     % Based on its assessment, the LLM returns a structured modeling strategy, such as: Use GRU4Rec to generate structured user embedding.

%     \item\textbf{Final Ranking.} In the final step, the device-side agent performs ranking over the retrieved candidate set by integrating both the semantic user embedding and the structured user embedding. These two embeddings capture complementary aspects of user preference: the semantic embedding reflects intent inferred from the abstract, while the structured embedding captures sequential behavioral patterns. To determine their relative contribution, the LLM analyzes the clarity of the user’s query and the density and recency of their interaction history. A clear query paired with sparse or outdated behavior may lead to a heavier reliance on semantic representation, while rich and recent interaction data may prioritize the structured embedding. Based on this analysis, the LLM returns a fusion strategy specifying the weights assigned to each embedding. 
%     % A typical strategy output would be: Fuse structured and semantic embeddings with weights 0.7 and 0.3 respectively.
% \end{itemize}

% To operationalize the planning process, we distill the above analyses and constraints into a carefully designed prompt. This prompt guides the cloud-based LLM to generate an adaptive recommendation strategy by specifying the execution decisions for each module. The prompt clearly defines the task, provides necessary context from the user abstract, and enforces a structured output format to ensure consistency, interpretability, and ease of downstream parsing:
% We translate the above design considerations into a prompt-driven interface that enables the cloud-based LLM to generate adaptive, per-user recommendation strategies. This prompt explicitly defines the planning task, supplies the user abstract as input, and incorporates execution constraints in a structured output format. In doing so, we ensure that the generated strategies are both personalized and system-efficient.
% \begin{promptbox} 
% \textbf{Prompt for Strategy Planning:}\\
% \textit{\textcolor{purple}{Given the user abstract which contains query and behavioral summary, generate an adaptive recommendation strategy across four modules including (1) Semantic User Modeling, (2) Candidate Retrieval, (3) Structured User Modeling, and (4) Final Ranking.}}\\
% \\
% User abstract: \textcolor{teal}{$a_u$}\\
% \\
% \textbf{Tips for Decision Making:} \\ 
% \\
% For \textbf{Semantic User Modeling}, evaluate the informativeness of both the query and behavioral summary. Prioritize the query if it clearly conveys intent, and prioritize the behavioral summary if the user has a rich and recent interaction history. Assign weights accordingly to generate a high-quality semantic embedding.\\
% \\ 
% For \textbf{Candidate Retrieval}, select an appropriate number of relevant tag groups and determine a suitable candidate set size based on the clarity of user intent, behavioral signal strength, and domain characteristics. Use fewer tags and candidates when intent is clear and preferences are focused; expand when signals are sparse or the domain requires diversity. Choose from predefined tag counts {3, 5, 10, 20} and candidate sizes {500, 1000, 2000, 5000}, and assign weights to each tag group to guide retrieval allocation.\\
% \\
% For \textbf{Structured User Modeling}, first determine whether structured modeling is necessary by evaluating the quantity and recency of the user's interaction history. If the interactions are too sparse or outdated, skip this step to save resources. If modeling is warranted, choose an appropriate method from {SASRec, SR-GNN} based on behavioral characteristics: use SASRec when the user's interactions exhibit strong sequential patterns, and use SR-GNN when the behavior involves more complex, non-linear transitions that benefit from graph-based modeling.\\\\
% \\
% For \textbf{Final Ranking}, balance the semantic and structured embeddings for final ranking based on the clarity of the query and the quality of interaction history. Emphasize semantic embedding when the query is clear and history is sparse; prioritize structured embedding when behavior is dense and recent. Return weight values indicating their relative importance in the final scoring.\\
% \\
% \textbf{Output Format:} \\ 
% Semantic User Modeling - \{query: $\alpha$, behavior: $1-\alpha$\}\\
% Candidate Retrieval - \{$tag_1$: $N_1$, $tag_2$: $N_2$, ...\}\\
% Structured User Modeling - \{Model Name or None\}\\
% Final Ranking - \{semantic: $\beta$, structured: $1-\beta$\}
% \end{promptbox}

% To achieve this, each item $i \in \mathcal{I}$ is associated with an embedding vector $\textbf{e}_i \in \mathbb{R}^d$, which can be initialized by applying the cloud-based large language model $\Theta_l$ to the item's textual metadata $\text{text}(i)$ (e.g., title, description, tags), followed by mean pooling:
% \begin{equation}
%     \textbf{e}_i = \mathrm{AVG}(\Theta_l(text(i))).
% \end{equation}

% To support subsequent personalization tasks, all item embeddings $\{ \textbf{e}_i \}_{i \in \mathcal{I}}$ are stored in the cloud and made accessible through lightweight, low-latency query interfaces. This design avoids imposing large storage burdens on user devices, while still enabling the on-device agents to retrieve the necessary item embeddings as needed. In particular, it allows the edge-side system to compute structured user embeddings based on historical interactions and to re-rank the coarse candidate set $\mathcal{C}_u$ using both behavioral and semantic signals. By enabling on-demand access to item-level representations without full local replication, the framework balances efficiency, scalability, and privacy preservation.

% In summary, for each domain, we obtain a reduced item subset $\mathcal{I}_u' \subset \mathcal{I}_z$ that reflects either semantic relevance or spatial proximity , which is then passed to the candidate ranking stage. At this point, the cloud-side agent performs similarity scoring between the semantic user embedding $\textbf{e}_u$ and each item embedding $\textbf{e}_i$ in the reduced subset $\mathcal{I}_u'$. The relevance score of item $i$ is computed via inner product:
% \begin{equation}
% \hat{y}_i = \textbf{e}_u \cdot \textbf{e}_i, \quad \forall i \in \mathcal{I}_u'.
% \end{equation}
% We then select the top-$N$ items with the highest scores to form the coarse candidate set:
% \begin{equation}
% \mathcal{C}_u = \text{TopN} \left( \{ \hat{y}_i \mid i \in \mathcal{I}_u' \} \right).
% \end{equation}
% The candidate set $\mathcal{C}_u$, along with the corresponding item embeddings and metadata, is then transmitted to the device for subsequent fine-grained personalization and ranking.






% where $\phi_{exp}$ is another trainable adapter inspired by QLoRA, which enables SLM to produce high-quality, human-understandable explanations in resource-constrained settings. The adapter for explanation generation is optimized by aligning outputs of the adapted SLM and the powerful LLM: 
% \begin{equation}
%     \mathcal{L}_{exp} = l_{CE}(\mathcal{E}_u,\mathcal{E}'_u),
% \end{equation}
% where $l_{CE}$ is the cross entropy loss and $\mathcal{E}'_u$ is the output of LLM which take same inputs as the adapted SLM.




% To further align the generation quality of the abstract with cloud-level reasoning expectations, we introduce an adapter module $\phi_{abs}$ tailored for abstract generation. Inspired by the QLoRA architecture, this adapter is trained to enhance the expressiveness and factual precision of the SLM’s output under limited device-side resources. During training, we simulate the abstract generation process using both the lightweight on-device SLM $\Theta_s \oplus \phi_{abs}$ and the cloud-based LLM $\Theta_l$, and minimize the divergence between their outputs through a contrastive loss:

% \begin{equation}
% \mathcal{L}{abs} = l{CE}(a_u, a'_u),
% \end{equation}

% \noindent where $a_u = \Theta_s \oplus \phi_{abs}(q_u, \mathcal{X}_u)$ is the abstract generated by the adapted SLM, and $a'_u = \Theta_l(q_u, \mathcal{X}u)$ is the abstract generated by the full LLM using the same input. Here, $l{CE}$ denotes the cross-entropy loss applied over token sequences. This adapter training ensures that the SLM captures the same level of intent understanding and behavioral summarization as the LLM, thereby improving strategy planning quality without compromising privacy or efficiency.





% The optimization workflow of CDARA is presented in Algorithm \ref{alg:opt}. Specifically, We train the SLM adapters and item embeddings to align device-side behaviors with cloud-side reasoning, enable effective abstract generation and explainable outputs, and support accurate semantic matching for recommendation, all while preserving efficiency and personalization under resource constraints.


% The optimization workflow of LLMGPR is presented in Algorithm \ref{alg:opt}. At the very beginning (line 1), we regard Llama3-8b as the base large language model $\Theta$, which can be replaced by any other large language model if sufficient computational resources are available. After that, we initialize all trainable weights including the check-in sequencing adapter $\Theta^{'}_s$, the aggregation adapter $\Theta^{'}_a$, the POI embedding matrix $\textbf{E}_{poi}$, and the purpose embedding matrix $\textbf{E}_{pur}$ (line 2). Then, we obtain the sequence-specific LLM $\Theta_s$ and the aggregation-specific LLM $\Theta_a$ (line 3-4). On this basis, we first pre-train the sequencing adapter $\Theta^{'}_s$ and the POI embedding matrix $\textbf{E}_{poi}$ based on the purpose prediction loss $\mathcal{L}_{pur}(y'_p,y_p)$ using all short sequences and their corresponding purpose labels (lines 5-10). The sequencing adapter $\Theta^{'}_s$ and the POI embedding matrix $\textbf{E}_{poi}$ are further optimized by the POI prediction loss $\mathcal{L}_{poi}(y',y)$ (lines 11-16). To address the group check-in data sparsity and obtain a better task-specific LLM for learning the representation of check-in sequences, all check-in sequences are utilized including group and all individual check-in sequences.

% Subsequently, the aggregation adapter $\Theta^{'}_a$ is trained iteratively with group check-in sequences and corresponding individual check-in sequences of each group member (lines 17-29). In detail, for each group check-in sequence, the group representation is originally obtained by applying the sequence-specific LLM $\Theta_s$ to the group check-in sequence (line 19). After that, individual representations for group members are obtained by applying $\Theta_s$ to their respective check-in sequences (lines 20-23). These representations are then fed into the aggregation-specific LLM $\Theta_a$ (line 24), while the aggregated representation is utilized to enhance the group representation (line 25) and generate the recommendation results (line 26). Finally, the aggregation adapter is updated using the POI prediction loss $\mathcal{L}_{poi}(y',y)$ (line 27).



% % Training subjects:
% 1. adapter for abstract generation
% 2. adapter for explaniable recommendation
% 3. item embeddings



% To enable CDARA to perform personalized, efficient, and interpretable recommendations, we train three key components in a collaborative manner: (1) an adapter for user abstract generation, (2) an adapter for explainable recommendation, and (3) the item embedding matrix. These components serve distinct yet complementary roles in the recommendation pipeline.

% The abstract generation adapter equips the on-device small language model (SLM) with the ability to compress user intent and behavior into a concise, privacy-preserving summary. This abstract serves as the foundation for downstream strategy planning and semantic modeling.

% The explainable recommendation adapter enables the SLM to generate natural language rationales for the final recommendations, enhancing transparency and user trust. By aligning its outputs with those of a powerful cloud-based LLM, the SLM learns to produce high-quality, human-understandable explanations in resource-constrained settings.

% Finally, the item embedding matrix is jointly trained to capture semantic and behavioral signals by aligning with both the abstract-based semantic user representation and the structured interaction history. This alignment ensures that the retrieved and ranked candidates accurately reflect the user's current preferences.

% Together, these components form the backbone of CDARA’s collaborative intelligence: cloud and device agents jointly optimize different aspects of the recommendation process while respecting privacy and resource constraints.




% % 1. semantic user embedding Vs item embedding
% % 2. structured user embedding vs item embedding
% % 3. slm vs llm - 总结和可解释性

% The small language model is trained on the cloud side and deployed on the user's device.

% \begin{algorithm}
%   \caption{The optimization of CDARA.}
%   \label{alg:opt}
% \begin{algorithmic}[1]
%     \STATE Obtain the large language model $\Theta_l$;
%     \STATE Obtain the small language model $\Theta_s$;
%     \STATE Initialize the item embedding matrix $\textbf{E}_{\mathcal{I}}$
%     \STATE Initialize adapters $\phi_{abs}$ and $\phi_{exp}$ for abstract generation and explainable recommendation respectively;
%     \REPEAT
%         \FOR{$(q, \mathcal{X},y)\in\mathcal{D}$}
%             \STATE $a' = \Theta_s\oplus\phi_{abs}(q,\mathcal{X})$;
%             \STATE $a = \Theta_l(q,\mathcal{X})$;
%             \STATE Take a gradient step w.r.t $\mathcal{L}_{abs}(a',a)$ to update $\phi_{abs}$;
%             \STATE $\alpha, \beta, \pi = \Theta_l(a)$
%             \STATE $\textbf{e}^{sem} = \alpha \cdot AVG(\Theta_l(q_u)) + (1-\alpha) \cdot AVG(\Theta_l(b_u))$;
%             \STATE $\textbf{e}^{str} = f_{loc}(\mathcal{X})$;
%             \STATE $\textbf{e}_u = \lambda \cdot \textbf{e}_u^{\text{sem}} + (1 - \lambda) \cdot \textbf{e}_u^{\text{str}}$;
%             \STATE $y' = \textbf{E}_\mathcal{I}(\textbf{e})$;
%             \STATE Take a gradient step w.r.t $\mathcal{L}_{rec}(y',y)$ to update $\textbf{E}_\mathcal{I}$;
%             \STATE $\Lambda' = \Theta_s\oplus\phi_{exp}(\pi,\mathcal{R})$;
%             \STATE $\Lambda = \Theta_l(\pi,\mathcal{R})$;
%             \STATE Take a gradient step w.r.t $\mathcal{L}_{exp}(\Lambda',\Lambda)$ to update $\phi_{exp}$;
%         \ENDFOR
%     \UNTIL{convergence}
% \end{algorithmic}
% \end{algorithm}

% \subsection{Framework Overview}
% Figure X illustrates our proposed cloud-edge collaborative multi-agent framework for personalized recommendation. The end-to-end workflow is decomposed into multiple sub-tasks, each targeting a specific functional aspect of the recommendation process:

% \begin{enumerate}[leftmargin=*]
%     \item \textbf{Intent Classification:} Determine the recommendation domain based on the user query $q_u$.
%     \item \textbf{Prompt Construction:} Generate a structured and privacy-preserving prompt $a_u$ using the user's profile $h_u$, context $k_u$, and interaction summary $\mathcal{X}_u$.
%     \item \textbf{Semantic User Modeling:} Use the cloud-based LLM to generate a semantic user embedding $\textbf{e}_u^{sem}$ from the prompt $a_u$.
%     \item \textbf{Candidate Retrieval:} Use the semantic embedding $e_u^{sem}$ to retrieve a coarse candidate set $\mathcal{C}_u$ from the domain-specific item subset $\mathcal{I}_d$.
%     \item \textbf{Behavioral Modeling:} Use on-device interaction history $\mathcal{X}_u$ to compute a structured user embedding $\textbf{e}_u^{\text{str}}$.
%     \item \textbf{Fine Ranking:} Fuse $\textbf{e}_u^{sem}$ and $\textbf{e}_u^{str}$ to re-rank $\mathcal{C}_u$ and generate the final Top-$K$ recommendation list $\mathcal{R}_u$.
%     \item \textbf{Explanation Generation:} Optionally produce interpretable natural language explanations for the recommended items based on the ranking results and user representation.
%     \item \textbf{User State Update:} After the recommendation session is completed, update the user state with new contextual information and interaction records to support continual personalization.
% \end{enumerate}
% These sub-tasks are distributed across three specialized agents, which operate collaboratively across cloud and device environments to efficiently execute the full recommendation pipeline:
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Coordinator Agent (Device-side):} This agent serves as the central controller for the entire workflow. It receives the recommendation query $q_u$, classifies the corresponding intent domain (Task 1: Intent Classification), gathers relevant user-side information including profile $h_u$, context $b_u$, and interaction history $\mathcal{X}_u$, and constructs a structured, privacy-preserving prompt $p_u$ (Task 2: Prompt Construction). It also monitors subtask execution and coordinates data flow among agents throughout the process. After the recommendation process is completed, the Coordinator Agent is responsible for updating the user state with new contextual information and interaction records (Task 8: User State Update).

%     \item \textbf{Cloud Retrieval Agent (Cloud-side):} This agent is responsible for performing large-scale semantic retrieval. Upon receiving the prompt $q_u$, it uses a cloud-based large language model to generate a semantic user embedding $\textbf{e}_u^{\text{sem}}$ (Task 3: Semantic User Modeling), and uses this embedding to retrieve a coarse candidate set $\mathcal{C}_u$ from the appropriate domain-specific item subset $\mathcal{I}_d$ (Task 4: Candidate Retrieval).

%     \item \textbf{Ranking Agent (Device-side):} This agent conducts fine-grained personalization. It first computes a behavioral embedding $\textbf{e}_u^{str}$ from the user's interaction history $\mathcal{X}_u$ using a lightweight on-device model (Task 5: Behavioral Modeling), and then fuses this embedding with $\textbf{e}_u^{\text{sem}}$ to re-rank the coarse candidate set $\mathcal{C}_u$ and produce the final Top-$K$ recommendation list $\mathcal{R}_u$ (Task 6: Fine Ranking). Additionally, it optionally generates human-readable explanations for the recommended items (Task 7: Explanation Generation).
% \end{itemize}

% To fully leverage the complementary strengths of cloud and edge environments, our framework enables efficient parallel collaboration between agents. In particular, Semantic User Modeling (Task 3) and Behavioral Modeling (Task 5) are executed simultaneously, as they operate on independent data sources—cloud-side abstract prompts and device-side interaction histories, respectively. This parallel execution not only reduces inference latency, but also allows the system to exploit the cloud agent’s powerful LLM capabilities for semantic reasoning while preserving user privacy through on-device behavioral modeling. By decoupling tasks across the cloud and edge, the framework achieves scalable, low-latency, and privacy-aware personalized recommendation. The collaborative multi-agent design ensures that each component contributes specialized capabilities toward accurate and trustworthy recommendation results.


% \subsection{Coordinator Agent}
% The Coordinator Agent, deployed on the user device, is responsible for both initiating and concluding the recommendation process. It operates a lightweight large language model (LLM) locally to interpret the user query, identify the appropriate recommendation domain, and generate a privacy-preserving prompt that captures the user’s intent, profile, contextual information, and behavioral history. Upon completion of the recommendation session, the agent further updates the user’s local state with newly observed interactions and contextual signals, ensuring that future recommendations remain adaptive and personalized.


% % Done
% \subsubsection{Task 1 - Intent Classification}
% Upon receiving a recommendation query $q_u$, the Coordinator Agent leverages an on-device LLM to determine the target recommendation domain, including Music, Book, Movie, Sport, and POI. Instead of relying on brittle rule-based keyword matching, the agent prompts the LLM with a natural language query analysis instruction and expects a single domain label as output, denoted as $z_u$. This inferred intent not only guides the selection of the corresponding item subset $\mathcal{I}_z \subset \mathcal{I}$ for downstream retrieval, but also provides contextual grounding for the subsequent construction of the user description prompt. While we focus on five domains in this work, the framework is readily extensible to support additional or custom-defined domains with minimal adaptation. The corresponding prompt used for intent classification is shown below:
% \begin{promptbox}  
% \textbf{Intent Classification Prompt:}\\
% \textit{\textcolor{purple}{Your task is to determine the type of recommendation requested in the following user query:} \\
% User Query: \textcolor{teal}{$q_u$}\\
% \textcolor{black}{Return only one of the following domain labels as your answer:} 
% \{\textbf{Music}, \textbf{Book}, \textbf{Movie}, \textbf{Sport}, \textbf{POI}\}
% } 
% \end{promptbox}  


% % Done
% \subsubsection{Task 2 - Prompt Construction for Semantic Embedding}
% After identifying the recommendation domain $z_u$, the Coordinator Agent retrieves relevant user-side information based on the user ID, including the static profile $h_u$, contextual signals $b_u$, and the domain-specific interaction history $\mathcal{X}_u$. These components are then organized into a structured intermediate instruction prompt, which is passed to the on-device LLM $\Theta_{\text{local}}$. The role of this LLM is to synthesize the user's current intent, long-term interests, and behavioral signals into a high-level, privacy-preserving natural language description. This abstract description, denoted as $a_u$, serves as the input prompt for the cloud-side LLM, which subsequently generates the semantic user embedding used in coarse candidate retrieval. To preserve user privacy, the constructed prompt intentionally omits raw identifiers, exact timestamps, and item IDs. The first-stage instruction prompt is manually designed to ensure semantic consistency and controllable abstraction:
% \begin{promptbox}  
% \textbf{Prompt for Constructing User Abstract:}\\
% \textit{\textcolor{purple}{Given the following structured user-related information, your job is to generate a high-level, privacy-preserving description of the user. This description will be converted into an embedding vector and matched against item embeddings for initial candidate selection:}}\\
% \\
% User Profile: \textcolor{teal}{$h_u$}\\
% User-Item Interaction History: \textcolor{teal}{$\{\text{text}(i) \mid i \in \mathcal{X}_u\}$}\\
% User Query: \textcolor{teal}{$q_u$}\\
% Recommendation Domain: \textcolor{teal}{$z_u$}\\
% Context Signals: \textcolor{teal}{$b_u$}\\
% \\
% Please follow these guidelines: \\ 
% 1. Do not include raw item IDs, exact timestamps, or sensitive identifiers.\\
% 2. You may abstract or add noise to sensitive information (e.g., approximate geographic location).\\
% 3. Summarize both short-term preferences and long-term interests. 
% \end{promptbox}

% Here, $\{\text{text}(i) \mid i \in \mathcal{X}_u\}$ denotes a set of natural language descriptions for the items the user has interacted with in the past, covering key semantic attributes such as title, category, and tags. These item-level descriptions serve as the behavioral input to the on-device LLM and, together with other contextual fields, enable the generation of a user abstract $a_u$ that captures personalized intent in a privacy-preserving manner.





% % Done
% \subsubsection{Task 8 - User State Update}
% After the recommendation process is completed, the Coordinator Agent updates the local user state to support continual personalization. Specifically, it logs the current recommendation query $q_u$, the contextual conditions $k_u$ (e.g., time and location), and the final user interactions with the recommended items (e.g., clicks, skips, or dwell time). These updates are incorporated into the user's profile $h_u$ or appended to the interaction history $\mathcal{X}_u$, ensuring that future recommendations are informed by the most recent user behavior and contextual patterns. This update process is executed entirely on-device to preserve user privacy.



% % Done
% \subsection{Cloud Retrieval Agent}
% The Cloud Retrieval Agent, deployed on the server side, is responsible for generating a semantic user embedding and retrieving a coarse candidate set for recommendation. It takes as input the abstracted user description $a_u$, produced by the on-device LLM in response to the Prompt for Constructing User Abstract, and outputs a semantic embedding $e_u^{\text{sem}}$ along with a domain-specific candidate set $\mathcal{C}_u$. This agent enables large-scale, intent-aware retrieval while maintaining user privacy by operating only on the high-level abstraction $a_u$ without access to raw user data.

% % Done
% \subsubsection{Task 3 - Semantic User Modeling}
% Upon receiving the abstracted user description $a_u$, the Cloud Retrieval Agent encodes it into a semantic user embedding $e_u^{sem} \in \mathbb{R}^d$ using the pretrained large language model $\Theta_{cloud}$. Specifically, we tokenize $a_u$ and feed it into $\Theta_{cloud}$, then average the final-layer token embeddings to obtain a dense user representation:
% \begin{align}
%   e_u^{\text{sem}} = \mathrm{AVG}(\Theta_{cloud}(a_u)),
% \end{align}
% where $\mathrm{AVG}(\cdot)$ denotes mean pooling over the final-layer token representations produced by the cloud-based LLM $\Theta_{cloud}$.

% % Done
% \subsubsection{Task 4 - Candidate Retrieval}
% To identify a coarse set of candidate items for ranking, the Cloud Retrieval Agent performs similarity-based matching between the semantic user embedding $e_u^{\text{sem}}$ and item embeddings within the relevant recommendation domain. Each item $i \in \mathcal{I}$ is associated with an embedding vector $e_i \in \mathbb{R}^d$, which can be initialized by applying the cloud-based large language model $\Theta_{cloud}$ to the item's textual metadata (e.g., title, description, tags), followed by mean pooling:
% \begin{equation}
%     \textbf{e}_i = \mathrm{AVG}(\Theta_{cloud}(\text{text}(i))).
% \end{equation}
% This embedding strategy injects rich semantic information into item representations from the outset. To reduce the computational burden, we first filter the global item pool based on the predicted recommendation domain $z_u$, yielding a smaller domain-specific subset $\mathcal{I}_z \subset \mathcal{I}$. 


% While domain filtering significantly narrows the search space, computing similarities between the semantic user embedding $\textbf{e}_u^{sem}$ and all items in $\mathcal{I}_z$ can still be computationally expensive when the domain contains tens or hundreds of thousands of candidates. To address this, we introduce a group-based retrieval mechanism that partitions items into smaller clusters using domain-specific grouping strategies. Depending on the domain, items are grouped either semantically—based on shared textual attributes such as genres, tags, or categories—or spatially, according to geographic proximity.


% In semantically structured domains (i.e., music, book, movie, and sport), we construct group-level embeddings using the pretrained LLM $\Theta_{cloud}$. For each group $g_k$, we compile a representative textual summary $\text{text}(g_k)$ and encode it as:
% \begin{equation}
% \textbf{g}_k = \mathrm{AVG}(\Theta_{cloud}(\text{text}(g_k))),
% \end{equation}
% where $\mathrm{AVG}(\cdot)$ denotes mean pooling over the final-layer token embeddings. During retrieval, the semantic user embedding is matched against all group embeddings $\{\textbf{g}_k\}$ to compute similarity scores:
% \begin{equation}
% \hat{y}_{k} = \textbf{e}_u^{\text{sem}} \cdot \textbf{g}_k,
% \end{equation}
% where $\cdot$ denotes the inner product. We then select the top-$L$ most relevant groups and aggregate their items to form a filtered candidate subset $\mathcal{I}_u' \subset \mathcal{I}_z$.

% In the POI domain, where location is the dominant organizing factor, semantic abstraction is unnecessary. Instead, we define a spatial radius around the user's current coordinates and include only POIs within that geographic boundary. This location-based filtering also yields a reduced subset $\mathcal{I}_u'$ suitable for subsequent matching, without requiring group-level embeddings.

% In summary, for each domain, we obtain a reduced item subset $\mathcal{I}_u' \subset \mathcal{I}_z$ that reflects either semantic relevance or spatial proximity , which is then passed to the candidate ranking stage. At this point, the cloud-side agent performs similarity scoring between the semantic user embedding $\textbf{e}_u$ and each item embedding $\textbf{e}_i$ in the reduced subset $\mathcal{I}_u'$. The relevance score of item $i$ is computed via inner product:
% \begin{equation}
% \hat{y}_i = \textbf{e}_u \cdot \textbf{e}_i, \quad \forall i \in \mathcal{I}_u'.
% \end{equation}
% We then select the top-$N$ items with the highest scores to form the coarse candidate set:
% \begin{equation}
% \mathcal{C}_u = \text{TopN} \left( \{ \hat{y}_i \mid i \in \mathcal{I}_u' \} \right).
% \end{equation}
% The candidate set $\mathcal{C}_u$, along with the corresponding item embeddings and metadata, is then transmitted to the device for subsequent fine-grained personalization and ranking.

% To support subsequent personalization tasks, all item embeddings $\{ \textbf{e}_i \}_{i \in \mathcal{I}}$ are stored in the cloud and made accessible through lightweight, low-latency query interfaces. This design avoids imposing large storage burdens on user devices, while still enabling the on-device agents to retrieve the necessary item embeddings as needed. In particular, it allows the edge-side system to compute structured user embeddings based on historical interactions and to re-rank the coarse candidate set $\mathcal{C}_u$ using both behavioral and semantic signals. By enabling on-demand access to item-level representations without full local replication, the framework balances efficiency, scalability, and privacy preservation.


% % Done
% \subsection{Ranking Agent}
% The Ranking Agent, deployed on the user device, is responsible for generating the final personalized recommendation list based on the user’s interaction history $\mathcal{X}_u$, abstract semantic profile $a_u$, and the coarse candidate set $\mathcal{C}_u$ provided by the cloud. It performs three key tasks: constructing a structured user embedding from behavioral data, re-ranking the candidate items by integrating behavioral and semantic signals, and generating natural language explanations for the top-ranked recommendations. 

% % Done
% \subsubsection{Task 5 - Behavioral Modeling}
% To capture personalized behavioral preferences, the Ranking Agent derives a structured user embedding $\textbf{e}_u^{\text{str}}$ from the user's domain-specific interaction history $\mathcal{X}_u = \{(i_1, t_1), (i_2, t_2), \ldots, (i_M, t_M)\}$, where $i_m$ denotes the $m$-th interacted item and $t_m$ is the corresponding timestamp. This embedding jointly models long-term preferences and short-term behavioral signals, and is obtained via:
% \begin{equation}
% \textbf{e}_u^{\text{str}} = f_{\text{loc}}\left(\{(\textbf{e}_{i_m}, t_m)\}_{m=1}^M\right),
% \end{equation}
% where $f_{\text{loc}}(\cdot)$ represents the on-device behavioral modeling function, which can be instantiated using models such as LightGCN or a Transformer-based sequence encoder. Since this computation relies on item embeddings stored in the cloud, the device must first query these embeddings. To preserve user privacy, the request is obfuscated by mixing in a set of unrelated item IDs, ensuring the cloud cannot infer the user's true interaction history. 

% % Done
% \subsubsection{Task 6 - Fine Ranking}
% Given the structured embedding $\textbf{e}_u^{\text{str}}$ computed from user behavior and the semantic embedding $\textbf{e}_u^{\text{sem}}$ generated by the cloud-side LLM, the Ranking Agent fuses these two representations to capture both historical behavioral signals and intent-aware semantics. Specifically, we adopt a weighted linear fusion strategy:
% \begin{equation}
% \textbf{e}_u = \lambda \cdot \textbf{e}_u^{\text{sem}} + (1 - \lambda) \cdot \textbf{e}_u^{\text{str}},
% \end{equation}
% where $\lambda \in [0, 1]$ is a tunable hyperparameter that controls the relative contribution of semantic and behavioral signals. The fused user embedding is then compared with each item embedding $\textbf{e}_i$ in the candidate set $\mathcal{C}_u$ to compute final relevance scores:
% \begin{equation}
% \hat{y}_i = \textbf{e}_u \cdot \textbf{e}_i.
% \end{equation}
% The top-$K$ items based on the ranking scores form the final recommendation list:
% \begin{equation}
% \mathcal{R}_u = \text{TopK}\left( \{ \hat{y}_i \mid i \in \mathcal{C}_u \} \right).
% \end{equation}
% This lightweight fusion strategy enables efficient on-device ranking while preserving both global semantic intent and personalized behavioral context.


% % Done
% \subsubsection{Task 7 - Explanation Generation}
% To enhance transparency and foster user trust, the Ranking Agent optionally generates natural language explanations for the final recommendation results. Specifically, for the top-10 items in the ranked list $\mathcal{R}_u$, the agent leverages the on-device LLM $\Theta_{\text{local}}$ to produce fluent and personalized explanations. The generation process is guided by a structured prompt that combines the user's abstract representation and natural language descriptions of the recommended items, as illustrated below:

% \begin{promptbox}  
% \textbf{Explanation Generation Prompt:}\\
% \textit{\textcolor{purple}{Given the user's abstract description, generate a concise, natural language explanation for why each of the following items is recommended. Each explanation should reflect the user's preferences and the item's key features. Generate exactly one sentence for each item.}}\\
% \\
% User Abstract: \textcolor{teal}{$a_u$}\\
% Items: \textcolor{teal}{\{$\text{text}(i_1),\text{text}(i_2),\dots,\text{text}(i_{10})$\}}\\
% \end{promptbox}

% Here, $a_u$ denotes the user's abstract profile generated by the Coordinator Agent via the Prompt for Constructing User Abstract. Each $\text{text}(i)$ refers to the item's textual metadata, including key attributes such as category, functionality, genre, or location, depending on the recommendation domain.

% I am not sure about if I should describe the cloud-edge setting


% In addition to high-quality recommendations, the system can optionally generate user-controlled natural language explanations to clarify the rationale behind each suggestion.

% I am not sure about if I should describe the cloud-edge setting
% to be improved.
% \noindent\textbf{Personalized Recommendation via Cloud-Device Collaboration.} 
% We consider the problem of personalized recommendation in a cloud-device collaborative setting, where both the cloud and the device jointly execute the recommendation process through adaptive agent cooperation. Each user $u \in \mathcal{U}$ is associated with a recommendation query $q_u$ (e.g., “recommend a place for dinner nearby”) and a historical interaction sequence $\mathcal{X}_u = {(i_1, t_1), (i_2, t_2), \dots}$ that records the user's previous behaviors (e.g., clicks, visits, purchases) along with timestamps. The goal is to recommend a ranked list of items $\hat{\mathcal{Y}}_u$ from a large item corpus $\mathcal{I}$ that best matches the user's current intent and long-term preferences.
% 可解释性


% \noindent\textbf{Task Definition: Secure and Personalized Recommendation.}  
% Given a user $u$ with a natural language query $q_u$, static profile $h_u$, contextual signals $b_u$, and a domain-specific interaction history $\mathcal{X}_u$, the goal is to generate a Top-$K$ personalized recommendation list $\mathcal{R}_u$ from the corresponding item domain. The recommendation process should ensure data privacy by preventing exposure of sensitive user information (e.g., $h_u$, $\mathcal{X}_u$), operate efficiently with minimal response time, and maintain high recommendation accuracy tailored to both user intent and behavioral preferences. Moreover, the system should support one-click, fully automated recommendation generation, allowing users to receive high-quality results with minimal effort.

% CDARA is a cloud-device collaborative recommendation framework that dynamically adapts its recommendation strategy based on on the user's contextualized recommendation scenario including query specificity, behavior sparsity, and domain characteristics. As shown in Figure X, CDARA adopts a dual-agent architecture, where both the lightweight device-side agent and the cloud-side agent are powered by language models. These two agents cooperate to execute the recommendation process in a modular and context-aware manner. Instead of relying on a fixed pipeline, CDARA decomposes the recommendation task into multiple adaptive sub-tasks: (1) Abstract Generation (device); (2) Strategy Planning (cloud); (3) Sematic User Modeling (cloud); (4) Candidate Retrieval (cloud); (5) Structured User Modeling (device); (6) Final Ranking (device). These components are selectively activated and routed based on strategy plans tailored to each user and scenario.

% The recommendation cycle begins on the device. Upon receiving the user’s query, the device-side agent, powered by a small language model (SLM), first generates a user abstract based on the user’s query and historical interactions. This abstract consists of two components. The first is a sanitized query, which rephrases the original user query to remove personally identifiable or sensitive details while preserving intent. The second is a behavioral summary, which captures key behavioral signals such as interaction sparsity and provides a concise description of the user’s long-term preferences and short-term interests. The abstract is then transmitted to the cloud-side agent, which is powered by a large language model (LLM). Leveraging its strong natural language understanding and reasoning capabilities, the cloud agent performs strategy planning, determining how the recommendation task should be executed given the user’s query specificity, behavior sparsity, and domain characteristics. Based on the generated plan, the cloud agent performs semantic user modeling, producing a language-aware embedding that captures the user's intent and context. This embedding is then used for coarse candidate retrieval, matching against global item representations to obtain a semantically relevant candidate set. The retrieved candidates are returned to the device, where the agent performs structured user modeling based on local interaction history. The final recommendation list is generated through ranking, which may integrate both semantic and structured signals. 

% Specifically, we treat the interacted items in the user’s history as positive labels and sample negative items from the same domain to formulate a contrastive learning objective:
% \begin{equation}
% \mathcal{L}_{\text{REC}} = \sum_{J\in\mathcal{N}^-}log\sigma(\hat{y}_i - \hat{y}_j),
% \end{equation}




% For each training sample, we randomly sample $5$ negative items from the user's non-interacted items, and define the recommendation loss as:
% % \begin{equation}
% % \mathcal{L}_{\text{REC}} = -\log\sigma(\lambda_{i})+\frac{1}{5}\sum\limits_{j=1}^{5} \log(1-\sigma(\lambda_j))
% % \end{equation}
% \begin{equation}
% \mathcal{L}_{\text{REC}} = -(\log\sigma(\lambda_{i})+\log(1-\sigma(\lambda_j)))
% \end{equation}


% The overall training loss for item embedding is defined as:
% \begin{equation}
% \mathcal{L}_{\text{item}} = -\sum\limits_{n=1}^{N_{pos}}\left(\log\sigma(\alpha_{i})+\frac{1}{N_{neg}}\sum\limits_{j=1, j\neq i}^{N_{neg}} \log(1-\sigma(\alpha_j))\right)
% \end{equation}
% where 
% $N_{pos}$ is the number of positive samples, 
% $N_{neg}$ is the number of negative samples for each positive sample $p_i$ that are randomly drawn from users' non-interacted items.
% $\sigma(\cdot)$ is the sigmoid function, while
% $\lambda_i$ and $\lambda_j$ are respectively the scores assigned to the positive and negative samples.



% \begin{equation}
%   \mathcal{L}_{\text{match}} = l\left(\phi_i\left(\mathcal{X}_u\right), \mathcal{Y}_u\right),
% \end{equation}



% The \textbf{explanation generation adapter} $\phi_{\text{exp}}$ enhances the SLM’s ability to produce natural language explanations for final recommendations. It is optimized by aligning the SLM’s explanation output with that of the cloud LLM using the same prompt inputs:
% \begin{equation}
%     \mathcal{L}_{\text{exp}} = l_{\text{CE}}(\mathcal{E}_u, \mathcal{E}'_u),
% \end{equation}
% where $\mathcal{E}_u = \Theta_s \oplus \phi_{\text{exp}}(\pi_u, \mathcal{R}_u)$ and $\mathcal{E}'_u = \Theta_l(\pi_u, \mathcal{R}_u)$ are the explanations generated by the SLM and LLM respectively, based on the execution plan $\pi_u$ and the final recommendation list $\mathcal{R}_u$.


% This adapter training ensures that the abstract $a_u$ retains all decision-critical information necessary for strategy planning, thereby aligning the SLM’s summarization behavior with cloud-level reasoning expectations while maintaining privacy and efficiency.


% Together, these adapters ensure that device-side reasoning stays semantically consistent with cloud-side expectations, enabling privacy-aware, low-latency recommendation experiences without compromising quality or interpretability.


% \newsavebox{\promptboxbox}
% \newenvironment{promptbox}
%  {\begin{lrbox}{\promptboxbox}\begin{minipage}{\dimexpr\columnwidth-2\fboxsep}\itshape}
%  {\end{minipage}\end{lrbox}%
%   \par\medskip\noindent
%   \colorbox{bgcolor}{\usebox{\promptboxbox}}%
%   \par\medskip}


\usepackage[most]{tcolorbox} % 在导言区添加
\newtcolorbox{promptbox}{
  colback=gray!10,
  colframe=gray!80!black,
  fonttitle=\bfseries,
  title=Prompt,
  boxrule=0.4pt,
  arc=2pt,
  left=4pt,
  right=4pt,
  top=4pt,
  bottom=4pt
}

==> old_intro.tex <==
% Old introduction - cannot delete

% % Done
% In the modern era, personalized recommender systems have become essential tools for assisting users in discovering relevant content and making informed decisions across various platforms. Existing models such as those based on Recurrent Neural Networks (RNNs) \cite{xu2021long,han2021deeprec,long2023model}, Graph Neural Networks (GNNs) \cite{he2020lightgcn,gao2022graph}, and more recently, Large Language Models (LLMs) \cite{lin2024data,acharya2023llm,zhao2024llm} have achieved great success in academia and industry. Most of these models \cite{xu2021long,he2020lightgcn,lin2024data} are deployed in the cloud, where user data is transmitted to centralized servers for high-capacity inference as shown in Figure \ref{Fig:toyexample} (a). These cloud-based systems leverage powerful computational resources and large model capacities to deliver highly accurate recommendations. However, due to privacy concerns and transmission constraints, they are unable to directly access real-time user data, which hampers precise intent modeling. In addition, they often encounter computational bottlenecks with a large volume of user requests, making it difficult to allocate sufficient resources for personalized inference. 

% % Done
% In contrast, the rest works \cite{han2021deeprec,xia2022device,long2023model,zhao2024llm} deploy lightweight variants of the aforementioned models on user devices with techniques such as model compression and collaborative training, to enable on-device inference which is illustrated in Figure \ref{Fig:toyexample} (b). This design allows direct access to user data for efficient personalization and alleviates server-side computation load. Unfortunately, these methods are inherently constrained by the limited computational and memory resources of user devices, which hinders their ability to perform large-scale retrieval. Consequently, their recommendation accuracy often falls short compared to cloud-based counterparts.

% % Done
% To combine the large-scale retrieval capability of the cloud inference with direct data accessibility and resource decoupling enabled by on-device inference. recent research \cite{lv2025collaboration,yao2022device,yao2021device} has proposed hybrid recommendation frameworks which support cloud-device collaborative inference as demonstrated in Figure \ref{Fig:toyexample} (c). In this diagram, the cloud component is typically responsible for resource-intensive tasks that leverage globally available knowledge, while the on-device model focuses on lightweight, real-time computation using locally observed signals to support personalized inference. A representative example is LSC4Rec \cite{lv2025collaboration}, which integrates a cloud-based large language model with an on-device lightweight recommendation model (e.g., DIN \cite{zhou2018deep}). In this framework, the cloud module generates a candidate set and initial relevance scores based on globally available data. These are then transmitted to the user’s device, where the local model performs reranking using recent session behaviors and contextual information. The final recommendation result combines signals from both sides, allowing the system to achieve a balance between global generalization and local personalization.



% % Done
% Despite the promising design of existing cloud-device recommendation frameworks, three critical challenges remain unresolved:
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Neglecting User Heterogeneity.} Each user exist in a different state and exhibits distinct recommendation needs. For example, active users with rich and consistent interaction histories can benefit from fine-grained personalization that leverages long-term preferences and behavioral patterns. In contrast, inactive users or cold-start users lack sufficient behavioral signals for accurate modeling and therefore require more exploratory or diversity-promoting strategies to infer their interests. Additionally, users may differ in how clearly they express their intent. Some demonstrate strong, goal-directed behavior, while others engage in more ambiguous or exploratory interactions. However, existing cloud-device recommendation frameworks often overlook such variations in user state. As a result, they fail to deliver content that aligns with individual user needs, ultimately leading to reduced recommendation accuracy.
%     \item \textbf{Inefficient Cloud-Device Collaboration.} Existing cloud-device recommendation frameworks often rely on a static collaboration pattern, in which the cloud and device components perform fixed roles regardless of the task and context. This fixed execution flow can lead to inefficient resource utilization, since excessive cloud involvement increases overhead, whereas insufficient support from the cloud hampers performance when local resources are constrained. Without the ability to dynamically coordinate computational responsibilities based on user state, task complexity, or environmental conditions, current works fail to balance the needs of computational efficiency and recommendation quality.
%     \item \textbf{Lack of Interpretability.} Most existing frameworks act as black boxes where users receive recommendation results without understanding why specific items are presented. While some systems offer generic, post-hoc explanations, these are often superficial and fail to reflect the actual reasoning behind the recommendation process. The absence of transparent decision logic undermines user trust and restricts the system’s capacity to incorporate user feedback and enable further recommendations refinement. 
% \end{itemize}
% These challenges call for a more intelligent, flexible, and interpretable cloud-device recommendation framework that can dynamically adapt to diverse user scenarios, efficiently coordinate computational resources, and offer transparent, step-by-step explanations of its decision process.


% % Done
% Recent advances in large language models (LLMs) have inspired a new wave of multi-agent frameworks, where multiple LLM-driven agents collaborate to perform complex tasks such as web automation, software engineering, embodied control, and tool-based reasoning \cite{shu2023rah,wang2024macrec}. These systems demonstrate strong capabilities in decomposing high-level goals, coordinating task execution, and dynamically adapting to changing environments. Considering that these qualities align well with the challenges faced by cloud-device recommendation, we extend the LLM-based multi-agent paradigm to this setting, and propose CDARec, a novel \textbf{C}loud-\textbf{D}evice collaborative framework that leverages LLM-empowered \textbf{A}gents for adaptive \textbf{Rec}ommendation.

% % Done
% In detail, CDARec adopts a two-agent architecture, where a cloud-side large language model (LLM) agent and a on-device small language model (SLM) agent jointly execute the recommendation process. Unlike existing approaches that rely on a fixed recommendation pipeline, CDARec dynamically adjusts its decision-making process to accommodate diverse user needs. To achieve this, we design a strategy planning mechanism which utilizes the powerful cloud-side LLM to analyze contextual signals such as query specificity, behavior sparsity, and domain characteristics in a secure manner. It then synthesizes a personalized recommendation strategy that determines how to allocate modeling and inference tasks across cloud and device in a way tailored to the user’s current needs. This strategy-guided design allows CDARec to move beyond fixed recommendation pipelines, enabling flexible adaptation to diverse scenarios while improving both personalization effectiveness and resource coordination. In addition, CDARec naturally supports interpretable outputs since each step in the pipeline is planned and executed explicitly, with traceable reasoning paths and adaptive decisions. Our main contributions are summarized as follows:
% \begin{itemize}[leftmargin=*]
%     \item We propose CDARec, a novel cloud-device recommendation framework with a multi-agent architecture that integrates a cloud-based LLM and an on-device SLM for intelligent, flexible, and interpretable recommendations.

%     \item We design a strategy planning mechanism that adaptively allocates modeling and inference tasks between cloud and device based on user context and domain characteristics. This not only improves personalization accuracy and system efficiency, but also enhances interpretability by enabling transparent, step-by-step reasoning and explainable recommendation outputs.

%     \item We conduct extensive experiments on multiple real-world datasets. Results demonstrate that CDARec outperforms strong baselines in both accuracy and efficiency, validating its effectiveness under diverse user behaviors and recommendation domains.
% \end{itemize}
